Technical Report: Full Version of Analyzing and Optimizing Perturbation of DP-SGD Geometrically

Differential privacy (DP) has become a prevalent privacy model in a wide range of machine learning tasks, especially after the debut of DP-SGD. However, DP-SGD, which directly perturbs gradients in the training iterations, fails to mitigate the negative impacts of noise on gradient direction. As a result, DP-SGD is often inefficient. Although various solutions (e.g., clipping to reduce the sensitivity of gradients and amplifying privacy bounds to save privacy budgets) are proposed to trade privacy for model efficiency, the root cause of its inefficiency is yet unveiled. In this work, we first generalize DP-SGD and theoretically derive the impact of DP noise on the training process. Our analysis reveals that, in terms of a perturbed gradient, only the noise on direction has eminent impact on the model efficiency while that on magnitude can be mitigated by optimization techniques, i.e., fine-tuning gradient clipping and learning rate. Besides, we confirm that traditional DP introduces biased noise on the direction when adding unbiased noise to the gradient itself. Overall, the perturbation of DP-SGD is actually sub-optimal from a geometric perspective. Motivated by this, we design a geometric perturbation strategy GeoDP within the DP framework, which perturbs the direction and the magnitude of a gradient, respectively. By directly reducing the noise on the direction, GeoDP mitigates the negative impact of DP noise on model efficiency with the same DP guarantee. Extensive experiments on two public datasets (i.e., MNIST and CIFAR-10), one synthetic dataset and three prevalent models (i.e., Logistic Regression, CNN and ResNet) confirm the effectiveness and generality of our strategy.

==> abstract.tex <==
\begin{abstract}
	In recent years, federated learning (FL), which trains a global model across multiple local devices without data exchange, has become a prevalent machine learning technique to utilize data while preserving participants' privacy. Nevertheless, privacy can still be compromised by local parameter updates during the global aggregation. To address this problem, local differential privacy (LDP), which only sends the perturbed information to any third party, is a promising solution. Referred to as federated LDP-SGD, each local device only sends its perturbed parameters to the central server for global aggregation. However, its primary drawback is ineffective training process caused by overwhelming LDP noise, which consequently leads to low model utility. Although there are a few recent works which mitigate the impact of LDP noise on FL, their analysis is either not quantitative or limited in a single LDP mechanism.
	
	In this paper, we first propose an analytical framework that generalizes federated LDP-SGD and derives the impact of LDP noise on the federated training process. Based on this framework, we identify a new geometric perspective to optimize LDP noise and even help to speed up the convergence of federated LDP-SGD. Motivated by this, we then design a vectorized perturbation strategy \textit{LDPVec}, which perturbs both the magnitude and the direction of a gradient, and rearranges the direction of noise to make positive impact on the convergence. Both theoretical analysis and extensive experiments on two benchmark datasets, i.e., MNIST and CIFAR-10, and two machine learning models, i.e., logistic regression and multilayer perceptron, confirm the accuracy and effectiveness of both the framework and strategy.
\end{abstract}


==> conclusion.tex <==
\section{Conclusion}
\label{sec::con}
This work investigates the impact of LDP noise in federated LDP-SGD. For its convergence, we propose a general analytical framework to measure the impact of LDP noise on federated LDP-SGD, which also serve as a benchmark to compare federated LDP-SGD under various LDP mechanisms. For model utility, we propose \textit{LDPVec} to speedup the convergence while providing the same level of LDP protection, without changing LDP mechanism itself. Through theoretical analysis and extensive experiments, we confirm the generality and effectiveness of our framework and perturbation strategy under two commonly-used benchmark datasets.

%For the future work, we plan to study the optimal privacy budget allocation of \textit{LDPVec}, and extend \textit{LDPVec} to more complicated networks, such as ResNet. 

==> experiment.tex <==
\section{Experimental Evaluation}
\label{sec::exp}
This section empirically evaluates our analytical framework as well as the perturbation strategy \textit{LDPVec} in federated LDP-SGD. According to Section \ref{subsec::LDPVec}, we compare \textit{LDPVec} against the existing numerical perturbation under four state-of-the-art LDP mechanisms, namely, Laplace, Piecewise, Square wave and Gaussian. In addition, we also implement noise-free federated SGD as a benchmark to demonstrate the feasibility of \textit{LDPVec} in practice.
As for existing works on federated LDP-SGD, since they are confined to either relaxed LDP \cite{wei2020federated,kim2021federated} or one specific LDP mechanism \cite{10.1007/978-3-030-59410-7_33}, \textit{LDPVec} is orthogonal to them and thus comparison with them is unnecessary.

\begin{figure}[htbp]
	\centering
	\includegraphics[width=0.6\linewidth]{figure/experiment/1/benchmark.pdf}
	\caption{Analytical vs. Experimental Results on Distances from the Global Optima}
	\vspace{-0.2in}
	\label{fig::benchmark}
\end{figure}

\begin{figure*}[htbp]
	\begin{center}
		\includegraphics[width=0.35\textwidth]{figure/experiment/2/legend.pdf}\\
		\subfigure[Laplace ($\epsilon=0.1,E=5,N=500$)]{
			\includegraphics[width=0.3\linewidth]{figure/experiment/2/L1.pdf}
		}
		\subfigure[Laplace ($\epsilon=0.01,E=5,N=500$)]{
			\includegraphics[width=0.3\linewidth]{figure/experiment/2/L2.pdf}
		}
		\subfigure[Laplace ($\epsilon=0.001,E=5,N=500$)]{
			\includegraphics[width=0.3\linewidth]{figure/experiment/2/L3.pdf}
		}
		
		\subfigure[Piecewise ($\epsilon=0.1,E=5,N=500$)]{
			\includegraphics[width=0.3\linewidth]{figure/experiment/2/P1.pdf}
		}
		\subfigure[Piecewise ($\epsilon=0.01,E=5,N=500$)]{
			\includegraphics[width=0.3\linewidth]{figure/experiment/2/P2.pdf}
		}
		\subfigure[Piecewise ($\epsilon=0.001,E=5,N=500$)]{
			\includegraphics[width=0.3\linewidth]{figure/experiment/2/P3.pdf}
		}		
		
		\subfigure[Square ($\epsilon=0.1,E=5,N=500$)]{
			\includegraphics[width=0.3\linewidth]{figure/experiment/2/S1.pdf}
		}
		\subfigure[Square ($\epsilon=0.01,E=5,N=500$)]{
			\includegraphics[width=0.3\linewidth]{figure/experiment/2/S2.pdf}
		}
		\subfigure[Square ($\epsilon=0.001,E=5,N=500$)]{
			\includegraphics[width=0.3\linewidth]{figure/experiment/2/S3.pdf}
		}			
		
		\subfigure[Gaussian ($\epsilon=0.1,E=5,N=500$)]{
			\includegraphics[width=0.3\linewidth]{figure/experiment/2/G1.pdf}
		}
		\subfigure[Gaussian ($\epsilon=0.01,E=5,N=500$)]{
			\includegraphics[width=0.3\linewidth]{figure/experiment/2/G2.pdf}
		}	
		\subfigure[Gaussian ($\epsilon=0.001,E=5,N=500$)]{
			\includegraphics[width=0.3\linewidth]{figure/experiment/2/G3.pdf}
		}
	\end{center}
	\caption{Global Loss of Logistic Regression on MNIST under Various $\epsilon$, $E$ and $N$ }
	\label{fig::LRMnist}
\end{figure*}

\begin{figure*}[htbp]
	\setlength{\abovecaptionskip}{-0.0cm}  
	\begin{center}
		\includegraphics[width=0.35\textwidth]{figure/experiment/2/legend.pdf}\\			
		\subfigure[Laplace ($\epsilon=1,E=2,N=1000$)]{
			\includegraphics[width=0.3\linewidth]{figure/experiment/2/L5.pdf}
		}
		\subfigure[Piece ($\epsilon=1,E=2,N=1000$)]{
			\includegraphics[width=0.3\linewidth]{figure/experiment/2/P5.pdf}
		}
		\subfigure[Square ($\epsilon=1,E=2,N=1000$)]{
			\includegraphics[width=0.3\linewidth]{figure/experiment/2/S5.pdf}
		}
	\end{center}
	\caption{Global Loss of Multilayer Perceptron on CIFAR-10 }
	\label{fig::MLPCIFAR}
\vspace{-0.2in}
\end{figure*}

\subsection{Datasets and Models}
We use two common benchmark datasets for federated LDP-SGD: MNIST and CIFAR-10. 

\noindent
\textbf{MNIST.} This is a dataset of 70,000 gray-scale images (28x28 pixels) of handwritten digits from 0 to 9, commonly used for training and testing machine learning algorithms in image recognition tasks. As one of the de-facto benchmark for evaluating the performance of algorithms, it consists of 60,000 training images and 10,000 testing images, with an even distribution across the 10 digit classes.

\noindent
\textbf{CIFAR-10.} It is a dataset of 60,000 small (32x32 pixels) color images, divided into 10 distinct classes such as animals and vehicles, used for machine learning and computer vision tasks. It contains 50,000 training images and 10,000 testing images, with each class having an equal number of images.

As with the settings in Section \ref{subsec::case}, both datasets are distributed to each local device in a non-iid fashion such that each device contains samples of only two classes.  We adopt two machine learning models as local models, namely, the logistic regression (LR) \cite{yang2019federated} and multilayer perceptron (MLP) \cite{bishop1995neural}. The former is implemented in MATLAB and applied to MNIST, while the latter is implemented in Python on a friendly federated learning framework, Flower \cite{beutel2020flower} and applied to CIFAR-10. Their architectures and parameters are listed in Table \ref{tab::LR} and Table \ref{tab::MLP}, respectively. The loss function in both models is cross-entropy loss.

\subsection{Parameter Settings for Federated LDP-SGD}
In our experiments, we vary the privacy budget allocated to each round of federated LDP-SGD $\epsilon\in\left\{0.001,0.01,0.1,1\right\}$, and the number of local devices $N\in\left\{500,1000\right\}$. The total number of local iterations $T$ and the number of local iterations in each training round $E$ are varied in the set $\left\{500,5000\right\}$ and $\left\{2,5\right\}$, respectively. To evaluate our framework and strategy objectively, we use the basic SGD without any special optimization technique (e.g., momentum). The batch size $B$ is fixed to $32$, and the leaning rate is decayed by the following scheme $\eta^t=\frac{\eta^0}{1+t}$, where $\eta^0$ is chosen from the set $\left\{0.1,0.01\right\}$.

As for the privacy budget allocation, we evenly partition the privacy budget as per the number of dimensions in the gradient. According to \cite{zhang2022understanding}, we consistently use a constant clipping threshold $C$ throughout the training process. %Both implementations, deliberately adding the most tremendous noise to the gradient, aim to test the limit of our proposed perturbation strategy.

\begin{table}[tb]
	\centering
	\caption{Perturbation Comparison under Federated Logistic Regression: Testing Accuracy}
	\label{tab:accuracy}		
	\begin{tabular}{ccccccc}
		\Xhline{1pt}
		Dataset & Method & $\epsilon=0.001$ & $\epsilon=0.01$ & $\epsilon=0.1$  \\
		\Xhline{1pt}
		\multirow{8}*{\makecell{MNIST \\  (noise-free\\ 99.9\%)} }
		& Lap & 46.3\%& 46.3\%& 46.3\% \\
		& Pie & 53.6\%& 53.6\%& 53.6\%  \\
		& Squ & 54.8\%& 54.8\%& 54.8\% \\
		& Gau & 74.3\%& 74.3\%& 74.3\% \\	
		&Lap-Vec & 81.6\%& 75.1\%& 72.4\%  \\
		&Pie-Vec & 83.9\%& 77.3\%& 73.5\%  \\
		&Squ-Vec & 85.4\%& 79.2\%& 75.7\%  \\
		&Squ-Vec & 94.1\%& 87.8\%& 78.3\%	\\	
		\Xhline{1pt}								 			
	\end{tabular}
\vspace{-0.2in}
\end{table}

\subsection{Framework Validation}
In the first set of experiments, we implement federated LR on MNIST dataset to verify the accuracy of our analytical framework. We set $N=500$ local devices, $T=500$ total local iterations. In each training round, there are $E=5$ iterations and $\epsilon=0.1$ privacy budget. Since there are $T/E=100$ rounds, the overall privacy budget is $100*0.1=10$. Recall from Table \ref{tab::LR} that LR has a total of $7850$ parameters. As such, each parameter is allocated $1/7850\approx1.3\times 10^{-4}$ in each training round, which is extremely small.

We conduct 1,000 experiments under Laplace (``Lap''), Piecewise (``Pie''), Square wave (``Squ'') mechanisms and noise-free federated SGD (``SGD''), respectively and plot the mean distances between the current global model and the global optima in Figure \ref{fig::benchmark}. The legend labeled with ``Fra'' in the suffix means that this result is derived from our framework whereas that labeled with ``Exp'' is the experimental result. Within an acceptable error bound, our derivation matches those experimental results, which confirms the accuracy of our framework.

\subsection{Effectiveness of LDPVec}
In the second set of experiments, we verify the effectiveness of our perturbation strategy \textit{LDPVec}. In Figure \ref{fig::LRMnist}, we plot the global loss of LR on MNIST dataset, under no perturbation (i.e., blue line), numerical perturbation (i.e., red line), and vectorized perturbation by \textit{LDPVec} (i.e., yellow line). From Figures \ref{fig::LRMnist} (a)-(l), where the privacy budget in each training round varies from $0.1$ to $0.001$, we can observe that LDPVec can help federated LDP-SGD to converge as close to noise-free federated SGD as possible.
%we can observe that our perturbation strategy achieves almost the same performance as noise-free federated SGD in most cases. The only exception is Figure \ref{fig::LRMnist} (c), where the convergence is delayed by the Laplace noise as the Laplace noise at $\epsilon=0.00001$ is very large. Nevertheless, \textit{LDPVec} can still converge. 
As for comparison, the performance of four LDP mechanisms under numerical perturbation is disappointing. In most cases, the training process ceases to converge and stop faraway from the global optima, which means the negative impact of LDP noise overshadows the positive impact. %Even worse, in Figures \ref{fig::LRMnist} (e), (f), gradient exposure occurs and the whole training process fails. Obviously, these bad situations are also incurred by overwhelming LDP noise from the numerical perturbation. 
These results coincide with the test accuracy results in Table \ref{tab:accuracy}, where suffix ``-Vec'' means our perturbation strategy while those without it means numerical perturbation. %We list the test accuracy of this model without LDP noise in the most left column. As we can see, our perturbation strategy is very feasible and robust even under cases where the numerical perturbation fails.

%To test the limit of our strategy, in Figure \ref{fig::LRMnist} (j)-(k) we set the number of local parities $N=5$, and $E=2$ (i.e., noisy aggregation happens every two local iterations). In this extreme case of steeply declined number of local devices and surging occurrences of noise injection, we observe that federated LDP-SGD under the numerical perturbation cannot converge. On the other hand, although \textit{LDPVec} suffers from delayed convergence as in Figure \ref{fig::LRMnist} (c), the final converged model still achieves almost similar loss to federated SGD without noise.

To demonstrate the generality of \textit{LDPVec} in various machine learning applications, we also conduct similar classification tasks on CIFAR-10 with Multilayer Perceptron (MLP). Due to the extremely large number of parameters, we raise the privacy budget to $\epsilon=1$ per training round and increase the total local iterations to $T=5,000$. As shown in Figure \ref{fig::MLPCIFAR}, we obtain similar results to LR on MNIST dataset. As such, we can conclude that \textit{LDPVec} can speedup the convergence which is likely to fail under the numerical perturbation, and achieve acceptable utilities under various datasets and models. 

\begin{table}[h!]
	\centering
	\caption{Parameters for Logistic Regression on MNIST}
	\label{tab::LR}
	\begin{tabular}{c|c|c|c}
		\hline
		Layer & Weights & Biases & Total \\ \hline
		Output (10 classes) & $784 \times 10 = 7840$ & $1 \times 10 = 10$ & 7850 \\ \hline
	\end{tabular}
\vspace{-0.2in}
\end{table}


\begin{table}[ht]
	\centering
	\caption{MLP Architecture and Parameters on CIFAR-10.}	
	\label{tab::MLP}
	\begin{tabular}{@{}llr@{}}
		\toprule
		Layer & Description & Number of Parameters \\
		\midrule
		Input       & 3072 dimensions (32x32x3) & 0 \\
		Hidden      & 200 neurons, tanh activation & $(3072 + 1) \times 200 = 614,\!600$ \\
		Output      & 10 classes (CIFAR-10) & $(200 + 1) \times 10 = 2,\!010$ \\
		\midrule
		Total       & & $614,\!600 + 2,\!010 = 616,\!610$ \\
		\bottomrule
	\end{tabular}
\vspace{-0.2in}
\end{table}




==> framework.tex <==
\section{A General Analytical Framework for Federated LDP-SGD}
\label{sec::framework}
In this section, we propose an analytical framework to generally analyze the convergence of federated LDP-SGD. In what follows, Section \ref{subsec::overview} generalizes federated LDP-SGD tasks, based on which we further model the global aggregation in Section \ref{subsec::model}, while analyzing the convergence of federated LDP-SGD in Section \ref{subsec::framework}. Finally, Section \ref{subsec::case} presents a case study, where we demonstrate the implementation of our framework on federated logistic regression, under Laplace, Piecewise and Square wave mechanisms, respectively.

\subsection{Overview of Federated LDP-SGD}
\label{subsec::overview}
Let us assume there are $T$ iterations in total, and one global aggregation occurs per $E$ iterations. As such, there are $T/E$ rounds of federated LDP-SGD. As shown in Figure \ref{fig::overview}, each round of federated LDP-SGD has five stages and finally terminates at stage \ding{177}.
\begin{enumerate}[label=\circled{\arabic*}]
	\item \emph{Local Regular Iterations:} On receiving the current global model $\boldsymbol{w}^{t*}$, each local device first updates its local model $\boldsymbol{w}_k^t=\boldsymbol{w}^{t*}$, and then initiates $E-1$ times local SGD as $		\boldsymbol{w}^{t+i}_k=\boldsymbol{w}^{t+i-1}_k-\eta^{t+i-1}\tilde{\boldsymbol{g}}^{t+i-1}_k, i=1, 2, ..., E-1$.

	\item \emph{Local Noisy Iteration:} On the $E$-th iteration, the gradient of the $E$-th local SGD is added by one random LDP noise. Formally,
	\begin{equation}
	\begin{aligned}
		\boldsymbol{w}^{t+E*}_k&=\boldsymbol{w}_k^{t+E-1}-\eta^{t+E-1} \boldsymbol{g}_k^{t+E-1*}\\
		&=\boldsymbol{w}^{t+E-1}_k-\eta^{t+E-1}(\tilde{\boldsymbol{g}}^{t+E-1}_k+\boldsymbol{n}^{t+E-1}_k)
	\end{aligned}
	\label{equ::stage2}		
	\end{equation}
	\item  \emph{To Server:} The perturbed models $\left\{\boldsymbol{w}_k^{t+E*}|1\leq k\leq N\right\}$ are sent to the central server while the original models remain locally.
	\item  \emph{Global Aggregation:} On receiving perturbed models from all devices, the central server aggregates perturbed models to derive the current global model. Formally,
	\begin{equation}
		\boldsymbol{w}^{t+E*}=\sum_{k=1}^{N} p_k\boldsymbol{w}_k^{t+E*}
	\label{equ::stage4}
	\end{equation}
	\item  \emph{Global Broadcast:} The central server updates the global model to each local device for the next round of local iterations. Namely, $\boldsymbol{w}_k^{t+E}=\boldsymbol{w}^{t+E*}$.
	\item  \emph{Global Stop:} LDP-SGD terminates when a satisfactory global model is derived.
\end{enumerate}

\begin{figure}[htbp]
	\centering
	\includegraphics[width=1\linewidth]{figure/illustration/overview.pdf}
	\caption{Overview of Federated LDP-SGD.}
	\label{fig::overview}
\vspace{-0.1in}
\end{figure}

In a complete round of federated LDP-SGD (Stages \ding{172}-\ding{176}), Stages \ding{172}-\ding{173} are ``the local iterations'' and Stages \ding{174}-\ding{176} are ``the global update'', respectively. Obviously, the LDP noise added on the local iteration (i.e., Stage \ding{173}) directly impacts the convergence on the global aggregation (i.e., Stage \ding{175}). The current convergence is then passed on to the following local iterations via the global broadcast (i.e., Stage \ding{176}), which further feeds back to the future convergence. Since analyzing such feedback for LDP noise as a whole system is complex, we alternatively model federated LDP-SGD stage by stage.

\subsection{Model of Federated LDP-SGD}
\label{subsec::model}
As Stages \ding{174},\ding{176} and \ding{177} are already described in Section \ref{subsec::overview}, we turn our focus Stages \ding{172},\ding{173} and \ding{175}, namely, local iterations and the global aggregation. Let $\Gamma_E$ denote the set of global updates, i.e., $\Gamma_E=\left\{nE|n=1,2,...,T/E\right\}$. When $t+1\in \Gamma_E$, it is the time to perform the global update after one noisy local iteration. Otherwise, it is just a local iteration. For simplicity, we can generalize local iterations (i.e., Stages \ding{172} and \ding{173}) in the $k$-th device as:
\begin{equation}
\begin{aligned}
	\boldsymbol{w}_k^{t+1*}=
	\begin{cases}
		\boldsymbol{w}_k^t-\eta^t \tilde{\boldsymbol{g}}^t_k, & \mbox{if} \quad t+1\notin \Gamma_E \\
		\boldsymbol{w}_k^t-\eta^t (\tilde{\boldsymbol{g}}^t_k+\boldsymbol{n}^t_k), & \mbox{if} \quad t+1\in \Gamma_E
	\end{cases}
\end{aligned}
\label{equ::ModelLocalIteration}
\end{equation}
Following Equation \ref{equ::ModelLocalIteration}, the global aggregation at Stage \ding{175} (i.e., $t+1\in \Gamma_E$) is modeled as:
\begin{equation}
	\boldsymbol{w}^{t+1*}=\sum_{k=1}^{N} p_k\boldsymbol{w}^{t+1*}_k
\label{equ::GlobalAggregation}
\end{equation}
Applying Equation \ref{equ::ModelLocalIteration} to Equation \ref{equ::GlobalAggregation}, we have :
\begin{equation}
	\begin{aligned}
		\boldsymbol{w}^{t+1*}&=\sum_{k=1}^{N} p_k\boldsymbol{w}_k^{t+1*}=\sum_{k=1}^{N} p_k(\boldsymbol{w}^{t}_k-\eta^{t}(\tilde{\boldsymbol{g}}^{t}_k+\boldsymbol{n}^{t}_k))\\
		&=\sum_{k=1}^{N} p_k(\boldsymbol{w}^{t}_k-\eta^{t}\tilde{\boldsymbol{g}}^{t}_k)-\eta^{t}\underbrace{\sum_{k=1}^{N}p_k\boldsymbol{n}^{t}_k}_A
	\end{aligned}
\label{equ::GlobalUpdate}
\end{equation}

As indicated in Equation \ref{equ::GlobalUpdate}, in local iterations two essential terms, namely the gradient itself and the LDP noise, jointly determine the global aggregation at Stage \ding{175}. While the gradient can be derived from the loss function, the random noise itself cannot be modeled. On the other hand, the aggregation of LDP noise (Item A) seems to be described by \emph{Lindeberg–Lévy Central Limit Theorem} (CLT)\cite{duan2022utility}. However, since different local devices in FL may have different weights, i.e., $\left\{p_k|1\leq k\leq N\right\}$, the sampled noise $p_k\boldsymbol{n}^{t}_k$ is non-identically distributed. This violates the prerequisite of CLT. Fortunately, we establish the following lemma, which uses a virtual aggregation $\bar{p}\sum_{k=1}^{N}\boldsymbol{n}^{t}_k$ to replace Item A, where $\bar{p}=\frac{\sum_{k=1}^{N}p_k}{N}$.
\begin{lemma}
	 Item A has the same distribution as $\bar{p}\sum_{k=1}^{N}\boldsymbol{n}^{t}_k$.
\label{lem::replace}
\end{lemma}
\begin{proof}
Given $\tilde{\boldsymbol{g}}^{t}_k$, $\boldsymbol{g}_k^{t*}$ is only decided by the LDP mechanism and the privacy budget. Therefore, $\boldsymbol{n}^{t}_k=\boldsymbol{g}_k^{t*}-\tilde{\boldsymbol{g}}^{t}_k$ follows the same distribution. Suppose the \textit{pdf} function of $\boldsymbol{n}^{t}_k$ is $f(\boldsymbol{x})$. Then, we have:
\begin{equation*}
\begin{aligned}
	&\sum_{k=1}^{N} p_k \boldsymbol{n}^{t}_k\int_{-\infty}^{\boldsymbol{x}} f(\boldsymbol{n}^{t}_k)d\boldsymbol{n}^{t}_k=	\sum_{k=1}^{N} p_k \boldsymbol{n}\int_{-\infty}^{\boldsymbol{x}} f(\boldsymbol{n})d\boldsymbol{n} 
	\\=&\bar{p}N\boldsymbol{n}\int_{-\infty}^{\boldsymbol{x}} f(\boldsymbol{n})d\boldsymbol{n}=\bar{p}\sum_{k=1}^{N} \boldsymbol{n}^{t}_k\int_{-\infty}^{\boldsymbol{x}} f(\boldsymbol{n}^{t}_k)d\boldsymbol{n}^{t}_k,
\end{aligned}
\end{equation*}
by which our claim is proven.
\end{proof}

Since $\boldsymbol{n}^{t}_k$ is identically distributed, we can use CLT \cite{duan2022utility} to describe the above virtual aggregation, namely, $\bar{p}\sum_{k=1}^{N}\boldsymbol{n}^{t}_k$. The same model also describes Item A, as proven by Lemma \ref{lem::replace}. However, no existing study instructs the strict LDP mechanisms to solve $\boldsymbol{n}^{t}_k$ given the clipped gradient $\tilde{\boldsymbol{g}}^{t}_{k}$. Following the same approach as existing LDP-SGD works \cite{wei2020federated,kim2021federated,10.1007/978-3-030-59410-7_33}, given the clipped gradient $\tilde{\boldsymbol{g}}^t_k(\left\|\tilde{\boldsymbol{g}}^t_k\right\|\leq C)$, its normalized gradient is $\tilde{\boldsymbol{g}}'^{t}_{k}=\tilde{\boldsymbol{g}}^{t}_{k}\sqrt{d}/C (\left\|\tilde{\boldsymbol{g}}'^{t}_{k}\right\|\leq \sqrt{d})$. Referring to Section \ref{subsec::LDP}, we can produce the normalized LDP noise $\boldsymbol{n}'^{t}_{k}$. While the normalized noise $\boldsymbol{n}'^{t}_{k}$ guarantees that the normalized perturbed gradient  $\boldsymbol{g}'^{t*}_{k}=\tilde{\boldsymbol{g}}'^{t}_{k}+\boldsymbol{n}'^{t}_{k}$ follows LDP, $\boldsymbol{n}^{t}_{kz}=\boldsymbol{n}'^{t}_{kz}C/\sqrt{d}$ guarantees that the perturbed gradient $\boldsymbol{g}^{t*}_{kz}=\tilde{\boldsymbol{g}}^{t}_{kz}+\boldsymbol{n}^{t}_{kz}$ also follows LDP, as guaranteed by the following lemma.

Since $\boldsymbol{n}^{t}_k$ is identically distributed, we can use CLT \cite{duan2022utility} to describe its aggregation, namely, $\sum_{k=1}^{N}\boldsymbol{n}^{t}_k$. However, there is no existing study on generally solving $\boldsymbol{n}^{t}_k$ given the clipped gradient $\tilde{\boldsymbol{g}}^{t}_{k}$. Following the same approach as analyzing existing LDP mechanisms (see Section \ref{subsec::LDP}), we first normalize the clipped gradient into $\left[-1,1\right]^d$, i.e.,  $\tilde{\boldsymbol{g}}'^{t}_{kz}=\tilde{\boldsymbol{g}}^{t}_{kz}\sqrt{d}/C$. If the normalized noise $\boldsymbol{n}'^{t}_k$ guarantees that the normalized perturbed gradient  $\boldsymbol{g}'^{t*}_k=\tilde{\boldsymbol{g}}'^{t}_k+\boldsymbol{n}'^{t}_k$ follows LDP, $\boldsymbol{n}^{t}_k=\boldsymbol{n}'^{t}_kC/\sqrt{d}$ guarantees that the perturbed gradient $\boldsymbol{g}^{t*}_{k}=\tilde{\boldsymbol{g}}^{t}_{k}+\boldsymbol{n}^{t}_{k}$ also follows LDP, as guaranteed by the following lemma.


Since $\boldsymbol{n}^{t}_k$ is identically distributed, we can use CLT \cite{duan2022utility} to describe its aggregation, namely, $\sum_{k=1}^{N}\boldsymbol{n}^{t}_k$. However, there is no existing study on generally solving $\boldsymbol{n}^{t}_k$ given the clipped gradient $\tilde{\boldsymbol{g}}^{t}_{kz} \in [-\frac{C}{\sqrt{d}},\frac{C}{\sqrt{d}}]$. Following the same approach as analyzing existing LDP mechanisms (see Section \ref{subsec::LDP}), we first normalize the clipped gradient into $\left[-1,1\right]$, i.e.,  $\tilde{\boldsymbol{g}}'^{t}_{kz}=\tilde{\boldsymbol{g}}^{t}_{kz}\sqrt{d}/C$. If the normalized noise $\boldsymbol{n}'^{t}_{kz}$ guarantees that the normalized perturbed gradient  $\boldsymbol{g}'^{t*}_{kz}=\tilde{\boldsymbol{g}}'^{t}_{kz}+\boldsymbol{n}'^{t}_{kz}$ follows LDP, $\boldsymbol{n}^{t}_{kz}=\boldsymbol{n}'^{t}_{kz}C/\sqrt{d}$ guarantees that the perturbed gradient $\boldsymbol{g}^{t*}_{kz}=\tilde{\boldsymbol{g}}^{t}_{kz}+\boldsymbol{n}^{t}_{kz}$ also follows LDP, as guaranteed by the following lemma.

Since $\boldsymbol{n}^{t}_k$ is independent and identically distributed, we can use CLT \cite{duan2022utility} to describe the above virtual aggregation, namely, $\sum_{k=1}^{N}\boldsymbol{n}^{t}_k$. However, there is no existing study on solving $\boldsymbol{n}^{t}_k$ given the clipped gradient $\tilde{\boldsymbol{g}}^{t}_{k}$. Following the same approach as analyzing existing LDP mechanisms (see Section \ref{subsec::LDP}), we first normalize the clipped gradient into $\left[-1,1\right]^d$, i.e.,  $\tilde{\boldsymbol{g}}'^{t}_{kz}=\tilde{\boldsymbol{g}}^{t}_{kz}\sqrt{d}/C$. If the normalized noise $\boldsymbol{n}'^{t}_k$ can guarantee that the normalized perturbed gradient  $\boldsymbol{g}'^{t*}_k=\tilde{\boldsymbol{g}}'^{t}_k+\boldsymbol{n}'^{t}_k$ satisfies $\epsilon$-LDP, $\boldsymbol{n}^{t}_k=\boldsymbol{n}'^{t}_kC/\sqrt{d}$ will guarantee that the perturbed gradient $\boldsymbol{g}^{t*}_{k}=\tilde{\boldsymbol{g}}^{t}_{k}+\boldsymbol{n}^{t}_{k}$ also satisfies $\epsilon$-LDP, as is guaranteed by the following lemma.
\begin{lemma}
	Let $\mathcal{M}: D\to R$ be a $(\epsilon,\delta)$-locally differentially private mechanism, and $f: J\to D$ be a linear mapping. Then $\mathcal{M}(f): J\to R$ is also $(\epsilon,\delta)$-locally differentially private.
	\label{lem::linear}
\end{lemma}
\begin{proof}
	For any pair of original data $\boldsymbol{g}'_i, \boldsymbol{g}'_j\in D$, any perturbed data $\boldsymbol{g}'^*\in R$ and their respective linear mapping $\boldsymbol{g}_i=f(\boldsymbol{g}'_i)$, $\boldsymbol{g}_j=f(\boldsymbol{g}'_j)$, $\boldsymbol{g}^*=f(\boldsymbol{g}'^*)$, we have:
	\begin{equation}
		\begin{aligned}
			&\Pr\left(f(\mathcal{M}(\boldsymbol{g}'_i))=\boldsymbol{g}^*\right)=\Pr\left(\mathcal{M}(\boldsymbol{g}'_i)=\boldsymbol{g}'^*\right)\\&\leq \exp(\epsilon)\Pr\left(\mathcal{M}(\boldsymbol{g}'_j)\right)+\delta=\exp(\epsilon)\Pr\left(f(\mathcal{M}(\boldsymbol{g}'_j))=\boldsymbol{g}^*\right)+\delta
		\end{aligned}
		\label{equ::post}
	\end{equation}
	Then we prove the equivalency of $f(\mathcal{M}(\boldsymbol{g}'_i))$ and $\mathcal{M}(\boldsymbol{g}_i)$. Suppose $f(\boldsymbol{x})=c\boldsymbol{x}$, we have:
	\begin{equation}
		\begin{aligned}
			f(\mathcal{M}(\boldsymbol{g}'_i))=f(\boldsymbol{g}'_i+\boldsymbol{n}'_i)=c\boldsymbol{g}'_i+c\boldsymbol{n}'_i=\boldsymbol{g}_i+\boldsymbol{n}_i=\mathcal{M}(\boldsymbol{g}_i)
		\end{aligned}
		\label{equ::equiv}
	\end{equation}
	Applying Equation \ref{equ::equiv} to Equation \ref{equ::post}, we have $		\Pr\left(\mathcal{M}(\boldsymbol{g}_i)=\boldsymbol{g}^*\right)\leq \exp(\epsilon)\Pr\left(\mathcal{M}(\boldsymbol{g}_j)=\boldsymbol{g}^*\right)+\delta$
	, by which this lemma is proven.
\end{proof}

 Suppose    $\boldsymbol{\mu}^t:\left\{\boldsymbol{\mu}^t_{z}=\mathbb{E}\left(\boldsymbol{n}'^{t}_{kz}\right)|1\leq z\leq d\right\}$ and $\boldsymbol{\sigma}^t:\left\{{\boldsymbol{\sigma}^t_{z}}^2=\mathbb{E}\left({\boldsymbol{n}'^{t}_{kz}}^2\right)-\mathbb{E}^2\left(\boldsymbol{n}'^{t}_{kz}\right)|1\leq z\leq d\right\}$, the following theorem derives Item A with a Gaussian distribution.
\begin{theorem}
 $\mathcal{N}(\frac{C\bar{p}_kN}{\sqrt{d}}\boldsymbol{\mu}^t,\frac{C^2\bar{p}_k^2N}{d}{{\boldsymbol{\sigma}^t}^2})$ is the distribution of Item A.
\end{theorem}
\begin{proof}
	For $\forall k$, $\boldsymbol{n}'^{t}_k$ are independent and identically distributed (i.i.d.) random variables. As per \emph{Lindeberg–Lévy Central Limit Theorem} \cite{SHANTHIKUMAR1984153,book,duan2022utility}, the following probability always holds if $N\rightarrow\infty$:
	\begin{equation}
		\begin{aligned}
			&\Pr\left(\frac{\sum_{k=1}^{N} \boldsymbol{n}'^{t}_{kz}-N\boldsymbol{\mu}^t_{z}}{\sqrt{N}{\boldsymbol{\sigma}^t_{z}}}\leq X\right)= \Pr\left(\frac{\frac{\sqrt{d}}{C}\sum_{k=1}^{N} \boldsymbol{n}^{t}_{kz}-N\boldsymbol{\mu}^t_{z}}{\sqrt{N}{\boldsymbol{\sigma}^t_{z}}}\leq X\right)\\=& \Pr\left(\frac{\sum_{k=1}^{N} \boldsymbol{n}^{t}_{kz}-\frac{CN}{\sqrt{d}}\boldsymbol{\mu}^t_{z}}{\sqrt{\frac{N}{d}}C{\boldsymbol{\sigma}^t_{z}}}\leq X\right)\\=& \Pr\left(\frac{\bar{p}_k\sum_{k=1}^{N} \boldsymbol{n}^{t}_{kz}-\frac{C\bar{p}_kN}{\sqrt{d}}\boldsymbol{\mu}^t_{z}}{\sqrt{\frac{N}{d}}\bar{p}_kC{\boldsymbol{\sigma}^t_{z}}}\leq X\right)
			=\int_{-\infty}^{X} \phi(x)dx,
		\end{aligned}
		\label{equ::normal}
	\end{equation}
	where $\phi(x)$ is the \textit{pdf} of the standard Gaussian distribution $\mathcal{N}(0,1)$. Therefore, $\lim\limits_{N\rightarrow\infty}\frac{\bar{p}_k\sum_{k=1}^{N} \boldsymbol{n}^{t}_{kz}-\frac{C\bar{p}_kN}{\sqrt{d}}\boldsymbol{\mu}^t_{z}}{\sqrt{\frac{N}{d}}C\bar{p}_k{\boldsymbol{\sigma}^t_{z}}}$ follows standard normal distribution. Then we derive the distribution of $\lim\limits_{N\rightarrow\infty}\bar{p}_k\sum_{k=1}^{N} \boldsymbol{n}^{t}_{kz}$ as $			\lim\limits_{N\rightarrow\infty}\bar{p}_k\sum_{k=1}^{N} \boldsymbol{n}^{t}_{kz}\sim\mathcal{N}(\frac{C\bar{p}_kN}{\sqrt{d}}\boldsymbol{\mu}^t_{z},\frac{C^2\bar{p}_k^2N}{d}{{\boldsymbol{\sigma}^t_{z}}^2})$.
%	\begin{equation}
%		\begin{aligned}
%			\lim\limits_{N\rightarrow\infty}\bar{p}_k\sum_{k=1}^{N} \boldsymbol{n}^{t}_{kz}\sim\mathcal{N}(\frac{C\bar{p}_kN}{\sqrt{d}}\boldsymbol{\mu}^t_{z},\frac{C^2\bar{p}_k^2N}{d}{{\boldsymbol{\sigma}^t_{z}}^2})
%		\end{aligned}
%		\label{equ::NormalDimension}
%	\end{equation}
	Due to the independence of each dimension of the clipped gradient, we can further derive the distribution of $\lim\limits_{N\rightarrow\infty}\bar{p}_k\sum_{k=1}^{N} \boldsymbol{n}^{t}_{k}$:
	\begin{equation}
		\begin{aligned}
			\lim\limits_{N\rightarrow\infty}\bar{p}_k\sum_{k=1}^{N} \boldsymbol{n}^{t}_{k}\sim\mathcal{N}(\frac{C\bar{p}_kN}{\sqrt{d}}\boldsymbol{\mu}^t,\frac{C^2\bar{p}_k^2N}{d}{{\boldsymbol{\sigma}^t}^2})
		\end{aligned}
		\label{equ::Normal}
	\end{equation}
	As proven by Lemma \ref{lem::replace}, item A shares the same distribution as $\bar{p}_k\lim\limits_{N\rightarrow\infty}\sum_{k=1}^{N} \boldsymbol{n}^{t}_{k}$, by which this theorem is proven.
\end{proof}
From Equation \ref{equ::normal}, gradient clipping, which reduces both the expectation and the variance of LDP noise, effectively reduce the magnitude of the LDP noise. However, it remains unclear how LDP noise impacts on the convergence. Now that we have mathematically derived a complete round of federated LDP-SGD, it is ready to analyze its convergence.
\subsection{A General Analytical Framework for Federated LDP-SGD}
\label{subsec::framework}
Let a virtual\footnote{By "virtual", we mean that they do not physically exist in the FL training process but are much convenient in terms of convergence analysis.} global gradient $\tilde{\boldsymbol{g}}^t=\sum_{k=1}^{N}p_k\tilde{\boldsymbol{g}}^t_k=\sum_{k=1}^{N}p_k\nabla F_k(\boldsymbol{w}_k^t, S_k^t)$, a virtual global noise $\boldsymbol{n}^t=\sum_{k=1}^{N}p_k\boldsymbol{n}^{t}_k$, and a virtual global model $\boldsymbol{w}^t=\sum_{k=1}^{N}p_k\boldsymbol{w}^{t}_k$. Then a virtual global SGD of federated LDP-SGD  $\boldsymbol{w}^{t+1*}=\sum_{k=1}^{N}p_k \boldsymbol{w}_k^t-\eta^t\sum_{k=1}^{N}p_k\tilde{\boldsymbol{g}}^{t*}_k=\boldsymbol{w}^t-\eta^t\left(\tilde{\boldsymbol{g}}^t+\boldsymbol{n}^{t}\right)$, and a virtual global model of federated SGD $\boldsymbol{w}^{t+1}=\sum_{k=1}^{N}p_k \boldsymbol{w}_k^t-\eta^t\sum_{k=1}^{N}p_k\tilde{\boldsymbol{g}}^{t}_k=\boldsymbol{w}^t-\eta^t\tilde{\boldsymbol{g}}^t$. Since $\nabla_k^t=\mathbb{E}(\tilde{\boldsymbol{g}}^{t}_k)$, we also have a virtual expectation of a global gradient $\nabla^t=\mathbb{E}(\tilde{\boldsymbol{g}}^t)=\sum_{k=1}^{N}p_k\nabla_k^t$. In general, the Euclidean distances between global models and the global optima (i.e., $\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^\star\right\|^2$ and $\left\|\boldsymbol{w}^{t+1}-\boldsymbol{w}^\star\right\|^2$) reflect the convergence states of federated LDP-SGD and federated SGD, respectively. Apparently, the smaller this distance is, the faster convergence the global model achieves. Their convergence difference (i.e., $\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^\star\right\|^2-\left\|\boldsymbol{w}^{t+1}-\boldsymbol{w}^\star\right\|^2$), on the other hand, can describe the impact of LDP noise on the global model, as presented by the following theorem.
\begin{theorem}
	Given $t+1\in \Gamma_E$, the impact of LDP noise on federated LDP-SGD can be measured as:
	\begin{equation}
		\begin{aligned}
			&\mathbb{E}\left(\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^\star\right\|^2\right)-\mathbb{E}\left(\left\|\boldsymbol{w}^{t+1}-\boldsymbol{w}^\star\right\|^2\right)\\=&-2\underbrace{\left\langle\boldsymbol{w}^t-\eta^t\nabla^t,\frac{C\bar{p}_kN}{\sqrt{d}}\boldsymbol{\mu}^t\right\rangle}_B\\&+\underbrace{\frac{C^2{\eta^t}^2\bar{p}_k^2N^2}{d}{\boldsymbol{\mu}^t}^2+\frac{C^2{\eta^t}^2\bar{p}_k^2N}{d}{{\boldsymbol{\sigma}^t}^2}}_C+2\underbrace{\left\langle\boldsymbol{w}^\star,\frac{C\bar{p}_kN}{\sqrt{d}}\boldsymbol{\mu}^t\right\rangle}_D
		\end{aligned}
		\label{equ::impact}
	\end{equation}
\end{theorem}
\begin{proof}
	From federated LDP-SGD, we have:
	\begin{equation}
		\begin{aligned}
			&\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^\star\right\|^2=\left\|\boldsymbol{w}^t-\eta^t\left(\tilde{\boldsymbol{g}}^t+\boldsymbol{n}^{t}\right)-\boldsymbol{w}^\star\right\|^2\\=&\left\|\boldsymbol{w}^t-\eta^t\tilde{\boldsymbol{g}}^t-\boldsymbol{w}^\star\right\|^2-2\langle\boldsymbol{w}^t-\eta^t\tilde{\boldsymbol{g}}^t-\boldsymbol{w}^\star,\boldsymbol{n}^{t}\rangle+{\eta^t}^2{\boldsymbol{n}^{t}}^2
		\end{aligned}
		\label{equ::LDPSGDGlobal}
	\end{equation}
	While for federated SGD, we have:
	\begin{equation}
		\left\|\boldsymbol{w}^{t+1}-\boldsymbol{w}^\star\right\|^2=\left\|\boldsymbol{w}^t-\eta^t\tilde{\boldsymbol{g}}^t-\boldsymbol{w}^\star\right\|^2
		\label{equ::SGDGlobal}
	\end{equation}
	Subtracting Equation \ref{equ::SGDGlobal} from Equation \ref{equ::LDPSGDGlobal}, we have:
	\begin{equation}
		\begin{aligned}
			&\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^\star\right\|^2-\left\|\boldsymbol{w}^{t+1}-\boldsymbol{w}^\star\right\|^2\\=&-2\langle\boldsymbol{w}^t-\eta^t\tilde{\boldsymbol{g}}^t-\boldsymbol{w}^\star,\boldsymbol{n}^{t}\rangle+{\eta^t}^2{\boldsymbol{n}^{t}}^2\\=&-2\underbrace{\langle\boldsymbol{w}^t-\eta^t\tilde{\boldsymbol{g}}^t,\boldsymbol{n}^{t}\rangle}_B+\underbrace{{\eta^t}^2{\boldsymbol{n}^{t}}^2}_C+2\underbrace{\langle\boldsymbol{w}^\star,\boldsymbol{n}^{t}\rangle}_D
		\end{aligned}
		\label{equ::difference}
	\end{equation}
	Recall that from Equation \ref{equ::Normal}, $\boldsymbol{n}^t$ approximates a Gaussian distribution $\mathcal{N}(\frac{C\bar{p}_kN}{\sqrt{d}}\boldsymbol{\mu}^t,\frac{C^2\bar{p}_k^2N}{d}{{\boldsymbol{\sigma}^t}^2})$. Given a variable $x$, its expectation $\mu$ and its variance $\sigma^2$, the expectation of item B is:
	\begin{equation}
		\mathbb{E}(B)=\langle\boldsymbol{w}^t-\eta^t\mathbb{E}(\tilde{\boldsymbol{g}}^t),\mathbb{E}(\boldsymbol{n}^{t})\rangle=\left\langle\boldsymbol{w}^t-\eta^t\nabla^t,\frac{C\bar{p}_kN}{\sqrt{d}}\boldsymbol{\mu}^t\right\rangle
		\label{equ::B}
	\end{equation}
	Given a variable $x$, its expectation $\mu$ and its variance $\sigma^2$, since $\mathbb{E}(x-\mu)^2=\mathbb{E}(x^2)-2\mu\mathbb{E}(x)+\mu^2=\mathbb{E}(x^2)-\mu^2=\sigma^2$, we have $\mathbb{E}(x^2)=\mu^2+\sigma^2$.
	On this basis, we derive the expectation of Item C:
	\begin{equation}
		\mathbb{E}(C)={\eta^t}^2\mathbb{E}({\boldsymbol{n}^t}^2)=\frac{C^2{\eta^t}^2\bar{p}_k^2N^2}{d}{\boldsymbol{\mu}^t}^2+\frac{C^2{\eta^t}^2\bar{p}_k^2N}{d}{{\boldsymbol{\sigma}^t}^2}
		\label{equ::C}
	\end{equation}
	For Item D, we have:
	\begin{equation}
		\mathbb{E}(D)=\langle\boldsymbol{w}^\star,\mathbb{E}(\boldsymbol{n}^{t})\rangle=\left\langle\boldsymbol{w}^\star,\frac{C\bar{p}_kN}{\sqrt{d}}\boldsymbol{\mu}^t\right\rangle
		\label{equ::D}
	\end{equation}
	Applying Equation \ref{equ::B}, \ref{equ::C} and \ref{equ::D} into Equation \ref{equ::difference}, we prove this theorem.
\end{proof}
Overall, a positive difference, i.e., $\mathbb{E}\left(\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^\star\right\|^2\right)>\mathbb{E}\left(\left\|\boldsymbol{w}^{t+1}-\boldsymbol{w}^\star\right\|^2\right)$, means that the convergence of federated LDP-SGD is slower than federated SGD. This perception is highly recognized by most existing works \cite{10.1007/978-3-030-59410-7_33,kim2021federated,wei2020federated,geyer2017differentially}. Zero difference, i.e., $\boldsymbol{\mu}^t=\boldsymbol{\sigma}^t=0$, means no LDP perturbation. The most interesting scenario is when the difference is negative, i.e., $\mathbb{E}\left(\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^\star\right\|^2\right)<\mathbb{E}\left(\left\|\boldsymbol{w}^{t+1}-\boldsymbol{w}^\star\right\|^2\right)$.

From Equation~\ref{equ::difference},the convergence difference is divided into three parts. Item B, the inner product between the noise-free global model and the noise itself, reflects the impact of LDP noise on the direction of convergence. Item C describes the impact of LDP noise on the scale of convergence. While item C is always non-negative, item B depends on the angle between the global gradient descent $\boldsymbol{w}^t-\eta^t\nabla^t$ and the global aggregation of noise $\boldsymbol{\mu}^t$. If the angle is acute, item B is negative and can reduce or even reverse the negative impact of item C. In other words, \textbf{LDP noise can sometimes speedup the convergence, rather than only slowing it down as perceived by most existing works.} Item D, however, shows that the introduction of LDP noise would definitely cause a bias to the global optima. In fact, the following corollary indicates that \textbf{federated LDP-SGD never reaches the global optima in a statistic sense.}
\begin{corollary}
The impact of LDP noise on federated LDP-SGD is convergent as follows:
\begin{equation}
\begin{aligned}
	&\lim_{t\to \infty}\mathbb{E}\left(\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^\star\right\|^2\right)-\mathbb{E}\left(\left\|\boldsymbol{w}^{t+1}-\boldsymbol{w}^\star\right\|^2\right)\\=&\frac{C^2{\eta^t}^2\bar{p}_k^2N^2}{d}{\boldsymbol{\mu}^t}^2+\frac{C^2{\eta^t}^2\bar{p}_k^2N}{d}{{\boldsymbol{\sigma}^t}^2}
\end{aligned}
\label{equ::impactinf}
\end{equation}
\end{corollary}
\begin{proof}
After sufficient iterations, federated SGD would finally converge to the global optima. As $\boldsymbol{w}^t-\eta^t\nabla^t$ models the non-LDP federated SGD, we have $\lim_{t\to \infty}\boldsymbol{w}^t-\eta^t\nabla^t\to\boldsymbol{w}^\star$. Applying this to Equation \ref{equ::impact}, we have Item B and Item D mutually canceled out. As such, this corollary is proven.
\end{proof}

Since this difference has a direct impact on the convergence, it can benchmark the utilities of various LDP mechanisms in federated LDP-SGD. In particular, $\boldsymbol{w}^t-\eta^t\nabla^t$ and $\boldsymbol{w}^\star$ can be derived according to the FL algorithms (e.g., FedAvg) and local datasets, while $\boldsymbol{\mu}^t$ and $\boldsymbol{\sigma}^t$ can be calculated from the LDP mechanisms. Although $\boldsymbol{w}^\star$ is unknown in practice, especially when the loss function is non-convex, it is a constant throughout the above derivation. Accordingly, we can calculate respective convergence differences in terms of respective LDP mechanism under FedAvg. The more negative the distance is, the faster convergence this mechanism achieves.

\subsection{A Case Study: Benchmarking LDP Mechanisms in Federated Logistic Regression}
\label{subsec::case}
To demonstrate our analytical framework, in this subsection we provide a case study on federated logistic regression \cite{yang2019federated}, where we benchmark the convergence of federated logistic regression under three state-of-the-art LDP mechanisms, namely, Laplace,
Piecewise and Square Wave mechanisms, in the global aggregation step, i.e., $t+1\in\Gamma_E$. We assume an MNIST \cite{lecun1998gradient} dataset (60,000 $28\times28$ images) distributed among $N=500$ devices in a non-iid fashion where each device contains 120 images of only two digits. 

For simplicity, we consider a binary classification task, where digits $0-4$ are labeled as "0", and digits $5-9$ are labeled as "1". Since each image has 784 pixels, the local model weight should have 785 dimensions (784 features plus 1 bias). Let $\boldsymbol{s}_{kj}:\left[1, \boldsymbol{s}_{kj}^1, \boldsymbol{s}_{kj}^2, ..., \boldsymbol{s}_{kj}^{783}, \boldsymbol{s}_{kj}^{784}\right]$ and $y_{kj}$ respectively denote one image and its label, and $\boldsymbol{w}_k^t:\left[\boldsymbol{w}_{k0}^t, \boldsymbol{w}_{k1}^t, ..., \boldsymbol{w}_{k783}^t, \boldsymbol{w}_{k784}^t\right]$ denote the local model. Then we have a linear combination $	v_{kj}={\boldsymbol{w}_k^t}^\top\boldsymbol{s}_{kj}=\sum_{z=1}^{785}\boldsymbol{w}_{kz}^t\boldsymbol{s}_{kj}^z$.
Given a sigmoid function $f(v)=\frac{1}{1+e^{-v}}$, we derive the probability of $\boldsymbol{s}_{kj}$ being identified as "0" and "1", respectively:
\begin{equation}
	\begin{aligned}
		\Pr(y_{kj}=1|\boldsymbol{w};\boldsymbol{s})=f(v_{kj}),\quad
		\Pr(y_{kj}=0|\boldsymbol{w};\boldsymbol{s})=1-f(v_{kj})		
	\end{aligned}
\end{equation}
Since there are 120 image in each device, we define the maximum likelihood function in terms of $\boldsymbol{s}_{kj}$:
\begin{equation}
	\begin{aligned}
		L(\boldsymbol{w};\boldsymbol{s}_{kj})&=\ln\Pr(y_{kj}|\boldsymbol{w};\boldsymbol{s}_{kj})\\&=y_{kj}\ln f(v_{kj})+(1-y_{kj})\ln(1-f(v_{kj}))
	\end{aligned}
\end{equation}
Obviously, the larger the likelihood, the more accurate the local model is. To derive the loss function $\mathit{l}(\boldsymbol{w};\boldsymbol{s}_{kj})=-L(\boldsymbol{w};\boldsymbol{s}_{kj})$, the local objective function of logistic regression is defined as follows:
\begin{equation}
	\begin{aligned}
		&F_k(\boldsymbol{w};S_{k})=\frac{1}{B}\sum_{j=1}^{B} \mathit{l} (\boldsymbol{w};s_{kj})\\&=-\frac{1}{B}\sum_{j=1}^{B}\left(y_{kj}\ln f(v_{kj})+(1-y_{kj})\ln(1-f(v_{kj}))\right)
	\end{aligned}
\end{equation}
where $B\leq 120$. For simplicity, we let $p_k=1/N=0.002$. Given $f'(v)=f(v)(1-f(v))$, the gradient $\boldsymbol{g}^t_k$ of the $t$-th local iteration is:
\begin{equation}
	\begin{aligned}
		\boldsymbol{g}^t_k&=\nabla F_k(\boldsymbol{w}^t_k;S_k)\\&=-\frac{1}{B}\sum_{j=1}^{B}\left(\frac{y_{kj}}{f(v_{kj})}-\frac{1-y_{kj}}{1-f(v_{kj})}\right)f'(v_{kj})\frac{\partial v}{\partial\boldsymbol{w}}\\&=-\frac{1}{B}\sum_{j=1}^{B}\left(y_{kj}(1-f(v_{kj}))-(1-y_{kj})f(v_{kj}) \right)\boldsymbol{s}_{kj}\\&=-\frac{1}{B}\sum_{j=1}^{B}\left(y_{kj}-f(v_{kj})\right)\boldsymbol{s}_{kj}=-\frac{1}{B}\sum_{j=1}^{B}\left(y_{kj}-f({\boldsymbol{w}_k^t}^\top\boldsymbol{s}_{kj})\right)\boldsymbol{s}_{kj}
	\end{aligned}
	\label{equ::CaseGradient}
\end{equation}
For simplicity, let $\boldsymbol{w}^t_k=\boldsymbol{w}^t=\boldsymbol{0}$. By setting $C=1.8$ and applying local datasets to Equation \ref{equ::CaseGradient}, we can derive:
\begin{equation}
	\begin{aligned}
		&\nabla^t=\sum_{k=1}^{N}p_k\nabla_k^t=\mathbb{E}(\tilde{\boldsymbol{g}}^t)=\mathbb{E}(\boldsymbol{g}^t)/\max \left\{1,\left\|\boldsymbol{g}_k^t\right\|/C\right\}\\&=-\frac{1}{500\times120}\sum_{k=1}^{500}\sum_{j=1}^{120}\frac{\left(y_{kj}-f({\boldsymbol{w}_k^t}^\top\boldsymbol{s}_{kj})\right)\boldsymbol{s}_{kj}}{\max \left\{1,\left\|\boldsymbol{g}_k^t\right\|/C\right\}}\\&=\frac{1}{60000}	\sum_{k=1}^{500}\sum_{j=1}^{120}\left(\frac{1}{2}-y_{kj}\right)\boldsymbol{s}_{kj}
	\end{aligned}
	\label{equ::Nabla}
\end{equation}
By setting $\eta^t=0.1$, we can derive $\boldsymbol{w}^t-0.1\nabla^t$.\footnote{We do not display $\nabla^t$ and $\boldsymbol{w}^t-0.1\nabla^t$ because each has 785 dimensions. } Let $\boldsymbol{w}^\star$ denote a well-trained model without LDP noise. In what follows, we demonstrate how to compare the utilities of federated logistic regression under different LDP mechanisms, while allocating privacy budget $\epsilon=0.1$ to each dimension.

\noindent
\textbf{Laplace mechanism.} First, we derive the expectation and the variance of the normalized noise $\boldsymbol{n}'^{t}_{kz}$. Namely,
\begin{equation}
	\begin{aligned}
		\boldsymbol{\mu}^t_{z}=\mathbb{E}\left(\boldsymbol{n}'^{t}_{kz}\right)=0,\
		{\boldsymbol{\sigma}^t_{z}}^2=\mathbb{E}\left({\boldsymbol{n}'^{t}_{kz}}^2\right)-\mathbb{E}^2\left(\boldsymbol{n}'^{t}_{kz}\right)=\frac{8}{\epsilon^2}=800
	\end{aligned}
	\label{equ::CaseLaplace}
\end{equation}
By applying Equation \ref{equ::CaseLaplace} to Equation \ref{equ::impact}, we have:
\begin{equation}
	\begin{aligned}
		&\mathbb{E}\left(\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^\star\right\|^2\right)-\mathbb{E}\left(\left\|\boldsymbol{w}^{t+1}-\boldsymbol{w}^\star\right\|^2\right)=-2\left\langle\boldsymbol{w}^t-\eta^t\nabla^t,\boldsymbol{0}\right\rangle\\+&\frac{C^2{\eta^t}^2\bar{p}_k^2N^2}{d}\sum_{z=1}^{785}{\boldsymbol{\mu}^t_z}^2+\frac{C^2{\eta^t}^2\bar{p}_k^2N}{d}\sum_{z=1}^{785}{{\boldsymbol{\sigma}_z^t}^2}+2\left\langle\boldsymbol{w}^\star,\boldsymbol{0}\right\rangle\approx 41.4
	\end{aligned}
	\label{equ::ImpactLap}
\end{equation}

\noindent
\textbf{Piecewise mechanism.} According to \cite{duan2022utility}, we have:
\begin{equation}
	\begin{aligned}
		\boldsymbol{\mu}^t_{z}&=\mathbb{E}\left(\boldsymbol{n}'^{t}_{kz}\right)=0\\
		{\boldsymbol{\sigma}^t_{z}}^2&=\mathbb{E}\left({\boldsymbol{n}'^{t}_{kz}}^2\right)-\mathbb{E}^2\left(\boldsymbol{n}'^{t}_{kz}\right)\\&=\frac{{\nabla_z^t}^2}{\exp(\epsilon/2)-1}+\frac{\exp(\epsilon/2)+3}{3(\exp(\epsilon/2)-1)^2}\approx513.4
	\end{aligned}
	\label{equ::CasePiece}
\end{equation}
Similar to Equation \ref{equ::ImpactLap}, we have:
\begin{equation}
	\begin{aligned}
		&\mathbb{E}\left(\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^\star\right\|^2\right)-\mathbb{E}\left(\left\|\boldsymbol{w}^{t+1}-\boldsymbol{w}^\star\right\|^2\right)\\=&-2\left\langle\boldsymbol{w}^t-\eta^t\nabla^t,\boldsymbol{0}\right\rangle+\frac{C^2{\eta^t}^2\bar{p}_k^2N^2}{d}\sum_{z=1}^{785}{\boldsymbol{\mu}^t_z}^2\\&+\frac{C^2{\eta^t}^2\bar{p}_k^2N}{d}\sum_{z=1}^{785}{{\boldsymbol{\sigma}_z^t}^2}+2\left\langle\boldsymbol{w}^\star,\boldsymbol{0}\right\rangle\approx 17.1
	\end{aligned}
	\label{equ::ImpactPiece}
\end{equation}

\noindent
\textbf{Square wave mechanism.} Based on \cite{duan2022utility}, we derive the corresponding expectation and variance of the normalized noise:
\begin{equation}
	\begin{aligned}
		\boldsymbol{\mu}^t_{z}&=\mathbb{E}\left(\boldsymbol{n}'^{t}_{kz}\right)=\frac{2b(e^{\epsilon}-1){\nabla_z^t}}{2be^{\epsilon/m}+1}+\frac{1+2b}{2(2be^{\epsilon/m}+1)}-{\nabla_z^t}\approx0.95\\
		{\boldsymbol{\sigma}^t_{z}}^2&=\mathbb{E}\left({\boldsymbol{n}'^{t}_{kz}}^2\right)-\mathbb{E}^2\left(\boldsymbol{n}'^{t}_{kz}\right)\\&=\frac{b^2}{3}+\frac{(2b+1)(b+1-3{\nabla_z^t}^2)}{3(2be^{\epsilon}+1)}-{\boldsymbol{\mu}^t_{z}}^2-2\boldsymbol{\mu}^t_{z}{\nabla_z^t}\approx1.25
	\end{aligned}
	\label{equ::CaseSquare}
\end{equation}
Accordingly, we have:
\begin{equation}
	\begin{aligned}
		&\mathbb{E}\left(\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^\star\right\|^2\right)-\mathbb{E}\left(\left\|\boldsymbol{w}^{t+1}-\boldsymbol{w}^\star\right\|^2\right)\\=&\underbrace{-2\left\langle\boldsymbol{w}^t-\eta^t\nabla^t,\frac{C\bar{p}_kN}{\sqrt{d}}\boldsymbol{\mu}^t\right\rangle}_B\\+&\underbrace{\frac{C^2{\eta^t}^2\bar{p}_k^2N^2}{d}\sum_{z=1}^{785}{\boldsymbol{\mu}^t_z}^2+\frac{C^2{\eta^t}^2\bar{p}_k^2N}{d}\sum_{z=1}^{785}{{\boldsymbol{\sigma}_z^t}^2}}_C+\underbrace{2\left\langle\boldsymbol{w}^\star,\boldsymbol{\mu}^t\right\rangle}_D\\\approx& -0.0387+0.0275+0.1143=0.103
	\end{aligned}
	\label{equ::ImpactSquare}
\end{equation}
Recall from Section \ref{subsec::framework} that a smaller convergence difference means better utility. Therefore, our benchmark reveals that Square wave provides the best convergence (i.e., $0.103$), followed by Piecewise (i.e., $17.1$), and then Laplace (i.e., $41.4$).

This case study also validates our observations in Section \ref{subsec::framework}. Item B in Equation \ref{equ::ImpactSquare}, a negative value $-0.0387$, does enhance the overall convergence while Item D, a positive value, does cause a bias from the global optima. Motivated by this, we next present a geometric perturbation strategy to enhance Federated LDP-SGD, without changing the LDP mechanism itself. 

==> introduction.tex <==
\section{introduction}
With the increasingly stringent legislation on personal data protection such as General Data Protection Regulation (GDPR) \cite{peukert2022regulatory}, federated learning (FL) \cite{yang2019federated}, a decentralized machine learning paradigm to train a global model across multiple local devices, has become increasingly popular over traditional centralized machine learning. %Besides, most FL frameworks, normally implementing prevalent deep learning algorithms (e.g., CNN) in local devices, are highly compatible with existing optimization techniques (e.g., mini-batch stochastic gradient descent (SGD) and its variants). Both high privacy and compatibility have been encouraging FL to embrace wider applications in practice.
However, recent studies show that the training process in FL, especially the disclosure of local model weights or gradients, can still leak private information and is thus vulnerable to various privacy attacks, including membership inference attacks \cite{melis2019exploiting,nasr2018comprehensive,shokri2017membership,yeom2018privacy}, attribute inference attacks \cite{jia2018attriguard,gong2018attribute}, and data extraction attacks \cite{carlini2021extracting,gong2021inversenet}. These attacks pose immediate threats to the wider adoption of FL in business sectors such as healthcare and finance where training data are sensitive.

To remedy this, local differential privacy (LDP), which sends the perturbed data to any third party while reserving original information locally, is embraced by both FL industry~\cite{tang2017privacy,abadi2016deep} and academia~\cite{duchi2013local}. Referred to as federated LDP-SGD, random noise is added to the local gradient or other derived local parameters before sent to the central server. As such, federated LDP-SGD effectively prevents privacy attacks on model parameters, as true parameters always remain locally.

However, a primary drawback of federated LDP-SGD is the ineffective training process caused by overwhelming noise, which extremely deteriorates model utility. There are a few works that attempt to improve utility but still have serious limitations. First, among various LDP mechanisms, only Gaussian mechanism, which merely provides relaxed privacy guarantee, is explored \cite{triastcyn2019federated,ruan2022private,geyer2017differentially,seif2020wireless,wei2020federated,kim2021federated,10.1007/978-3-030-59410-7_33}. Second, no prior works have theoretically modeled the impact of LDP noise on federated LDP-SGD, especially the training process. Last but not the least, LDP-SGD optimizations in prior works \cite{kim2021federated,10.1007/978-3-030-59410-7_33} commonly improve model utilities by reducing the number of model weights (i.e., increasing the privacy budget allocated to each weight), which however sacrifices the model architecture. %Therefore, they are harmful to structurally complicated algorithms (e.g., neural networks). Overall, existing works, even under relaxed privacy configuration, can only provide either trivial analysis on or limited model utilities to federated LDP-SGD.

In this paper, we address these limitations by first proposing an analytical framework that generalizes federated LDP-SGD and derives the impact of LDP noise on the federated training process, in terms of the difference of convergence. Then we show that this framework can serve as a benchmark to compare model utilities of federated LDP-SGD under various LDP mechanisms. An interesting observation is that while existing works all perceive LDP noise to damage the training process, our analysis points out that {\bf it can sometimes speedup the convergence of federated LDP-SGD} when the angle between the direction of the local model and that of the LDP noise is acute (i.e., the inner product of these two is positive). As such, existing LDP perturbation schemes become sub-optimal for federated LDP-SGD, as they only perturb the gradient as numerical values. Motivated by this, our second contribution is to design a geometric perturbation strategy \textit{LDPVec} to speedup the convergence of federated LDP-SGD. While retaining the same level of LDP protection, \textit{LDPVec} perturbs both the magnitude and the direction of a gradient, and rearranges the direction of LDP noise to make positive impact on the convergence. Without any change to the underlying LDP mechanism, it can serve as a general optimizer for federated LDP-SGD. In summary, our main contributions are as follows.
\begin{itemize}
	\item {To the best of our knowledge, this is the first general analytical framework to quantitatively study the impact of LDP noise on federated LDP-SGD. This framework can not only serve as a utility benchmark to compare various LDP mechanisms for federated LDP-SGD, but also point out the direction of future optimization.}
	\item {We propose a geometric perturbation strategy \textit{LDPVec} to speedup the convergence of Federated LDP-SGD, while still providing the same level of privacy guarantee.}
	\item {Extensive experiments on real datasets, popular machine learning models, and three state-of-the-art LDP mechanisms are conducted to validate the generality and effectiveness of both framework and strategy in federated LDP-SGD. All results unanimously show that the theoretical analysis is consistent with the experimental results, and our geometric perturbation strategy significantly speeds up the convergence in practice.}
\end{itemize}

The rest of this paper is organized as follows. In Section \ref{sec::related}, we review the related literature. Section \ref{sec::prob} introduces the basic concepts as well as the problem forumulation. Section \ref{sec::framework} presents the analytical framework for federated LDP-SGD while Section \ref{sec::stra} proposes the perturbation strategy \textit{LDPVec}. Experimental results are presented in Section \ref{sec::exp}, and conclusions are made in Section \ref{sec::con}. 

==> literature.tex <==
\section{Related Work}
\label{sec::related}
In this section, we review related works from three aspects: LDP, federated learning and their crossover works. On this basis, we also introduce the base of this work.
\subsection{Local Differential Privacy (LDP)}
Since Dwork \emph{et al.}~\cite{10.1007/11681878_14} first introduced the definition of \emph{differential privacy} (DP) and the first DP mechanism, i.e., Laplace mechanism, extensive DP-related works~\cite{dwork2014algorithmic,abadi2016deep,friedman2010data,mcsherry2007mechanism,wasserman2010statistical,kairouz2015composition} have been proposed. In particular, local differential privacy (LDP)~\cite{evfimievski2003limiting,raskhodnikova2008can,duchi2013local}, as the local variant of DP, provides more rigorous privacy preservation, and therefore draws much attention from many fields, including itemset mining~\cite{wang2018locally}, marginal release~\cite{cormode2018marginal, zhang2018calm}, time series data release~\cite{ye2021beyond}, graph data analysis~\cite{sun2019analyzing, ye2020towards, ye2021lfgdpr}, key-value data collection~\cite{ye2019privkv, gu2020pckv,ye2021privkvm}, and private learning~\cite{zheng2019bdpl, zheng2020protecting}.

The most relevant LDP works to our work are those on mean estimation. Dwork \emph{et al.}~\cite{10.1007/11681878_14} initially propose Laplace mechanism for LDP. Afterwards, several variants of Laplace mechanism, SCDF~\cite{soria2013optimal} and Staircase mechanism~\cite{geng2015staircase}, are proposed. As the perturbed values of these mechanisms range from negative to positive infinity, they are referred to as \emph{unbounded mechanisms} in this paper. On the other hand, \emph{bounded mechanisms} perturb values into a finite domain. Duchi \emph{et al.}~\cite{duchi2018minimax} present one whose outputs are binary while Wang \emph{et al.}~\cite{wang2019collecting} propose optimized ones, Piecewise mechanism and Hybrid mechanism. Besides, Li \emph{et al.}~\cite{li2020estimating} propose Square Wave mechanism, whose more concentrated perturbation is superior to above ones. To generalize all LDP mechanisms and measure their utilities, Duan \emph{et al.}~\cite{duan2022utility}, based on the Central Limit Theorem, propose a theoretical benchmark, which is used to model various LDP noise in this paper.

\subsection{Federated Learning}
Federated learning~\cite{konevcny2016federated,yang2019federated}, as a decentralized machine learning paradigm, allows participants to collectively train a global model without data transfer. Until now, a large body of FL works have been proposed, including efficiency improvement~\cite{sattler2019robust,hao2019efficient}, federated generative adversarial network~\cite{augenstein2019generative}, medical institution collaboration~\cite{sheller2020federated,sheller2018multi}, user profiling~\cite{hard2018federated}, benchmark design~\cite{he2020fedml}, and knowledge transfer~\cite{he2020group}.

Without loss of generality, we adopt the basic algorithm of FL, a.k.a, FedAvg \cite{mcmahan2017communication} for both analysis and experiments in this paper. As for privacy protection, we follow the common practice of existing works and adapt LDP to DP-SGD (LDP-SGD)~\cite{abadi2016deep}. The seminal work on FL convergence analysis~\cite{li2019convergence} provides us with a theoretical foundation to analyze the impact of LDP noise on FL. An open-source FL framework, known as Flower~\cite{beutel2020flower}, provides us with the experimental platform.

\subsection{Integrating LDP with FL (Federated LDP-SGD)}
As DP can defend federated learning against various inference attacks, their integration has led to flourishing outcomes in recent years. For example, Triastcyn \emph{et al.}~\cite{triastcyn2019federated} consider federated reinforcement learning under DP noise. Ruan \emph{et al.}~\cite{ruan2022private} provide a practical federated DP-SGD framework under secure multi-party computation protocols. Geyer \emph{et al.}~\cite{geyer2017differentially} study the client-level federated DP-SGD. Seif \emph{et al.}~\cite{seif2020wireless} apply federated DP-SGD to wireless systems.

Relevant to our work are those on utility analysis and enhancement. For convergence analysis, Wei \emph{et al.}~\cite{wei2020federated} investigate FL convergence under DP noise while Kim \emph{et al.}~\cite{kim2021federated} propose similar analysis under LDP noise. For utility enhancement, Liu \emph{et al.}~\cite{10.1007/978-3-030-59410-7_33} optimize federated machine learning under DP with top-k selection.

However, existing works have serious limitations. First, they are confined to Gaussian mechanism and thus lack of generality. Second, since these works are unable to accurately model the noisy training process, their analysis can only provide extremely loose bounds and thus make trivial conclusions, e.g., there is a trade-off between privacy budget and convergence rate. Third, their optimization is only effective under a large privacy budget, but leads to controversial results when applied to real world, where the privacy budget is usually limited.

So far, even under relaxed LDP, there is no existing work providing non-trivial analysis on federated LDP-SGD, let alone a general optimizer. Our work, on the other hand, accurately models the noisy training process as well as enhancing utility of federated LDP-SGD.


==> problem.tex <==
\section{Preliminaries and Problem Formulation}
\label{sec::prob}
In this section, we first introduce the preliminaries of LDP and FL, based on which we then formulate federated LDP-SGD into an optimization problem. Further utility analysis and enhancement of federated LDP-SGD are presented in Sections \ref{sec::framework} and \ref{sec::stra}, respectively. The most frequently-used notations in this paper are listed in Table \ref{tab::note}.
\begin{table}
	\caption{Notations}
	\renewcommand{\arraystretch}{1.2} %width
	\begin{center}
		\begin{tabular}{|c|c|}\hline
			\textbf{Symbol}&\textbf{Meaning} \\\hline
%			$N$&number of local devices \\\hline
%			$p_k$&weight of local dataset\\\hline
%			$F_k$&local objective function\\\hline
%			$T$&number of local iterations\\\hline
%			$E$&number of local iterations in each training round\\\hline
			$t$&the current local iteration\\\hline
%			$\eta^t$&the current learning rate \\\hline
			$\boldsymbol{w}_k^t$&the current local parameters\\\hline
			$\boldsymbol{w}^t$&the current global parameters \\\hline
			$\tilde{\boldsymbol{g}}_k^t$&the current local clipped gradient \\\hline
			$\boldsymbol{n}_k^t$&the current LDP noise \\\hline
			$\tilde{\boldsymbol{g}}_k^{t*}$&the current perturbed gradient \\\hline
		\end{tabular}
	\end{center}
	\label{tab::note}
\vspace{-0.2in}
\end{table}
\subsection{Local Differential Privacy}
\label{subsec::LDP}
 Suppose there are $N$ users, each of whom possesses a private value $g_k, 1\leq k\leq N$. Before sending to any third party, each original value is perturbed into a perturbed one $g_k^*$ by a perturbation mechanism $\mathcal{M}$. Given privacy budget $\epsilon>0$ indicating the privacy protection level, $\epsilon$-\emph{local differential privacy (LDP)} is formally defined as follows:
\begin{definition}
	\emph{($(\epsilon$,$\delta)$-local differential privacy)} A perturbation mechanism $\mathcal{M}: D\to R$ satisfies $\epsilon$-local differential privacy iff for any pair of original data $g_i, g_j\in D$ and any perturbed data $g^*\in R$, the following inequality always holds:
	\begin{equation*}
		\Pr\left(\mathcal{M}\left(g_i\right)=g^*\right)\leq\exp\left(\epsilon\right)\Pr\left(\mathcal{M}\left(g_j\right)=g^*\right)+\delta
	\end{equation*}
\end{definition}
In essence, LDP guarantees that given perturbed data $g^{*}$, it is unlikely for any third party to identify the data source with high confidence. On one hand, privacy budget $\epsilon$ controls the trade-off between privacy protection level and utility. Namely, a lower privacy budget means stricter privacy preservation and thus poorer utility, and vice versa. On the other hand, $\delta$ determines of the probability of not satisfying $\epsilon$ level of protection. That is, mechanism $\mathcal{M}$ satisfies $\epsilon$-LDP with probability $1-\delta$. In particular, $\delta=0$ is the strict LDP. Otherwise, it is the relaxed LDP.

Among various LDP mechanisms, the following four are state-of-the-art and are used for the experiments in Section \ref{sec::exp}. Since the first three follow the strict LDP while the last one follows relaxed LDP, they can represent all LDP mechanisms.

\noindent
\textbf{Laplace mechanism.} Given a value $g_k$ in the range of $[-1,1]$, the perturbed value is $g_k^*=g_k+Lap(2/\epsilon)$, where $Lap(\lambda)$ denotes a random variable that follows Laplace distribution with probability density function $f(x)=\frac{1}{2\lambda}\exp(-\frac{|x|}{\lambda})$.

As a classic LDP mechanism, the advantage of \emph{Laplace mechanism} \cite{10.1007/11681878_14} is its simplicity. Since its introduction in \cite{10.1007/11681878_14}, Laplace mechanism has evolved into a class of LDP mechanisms \cite{10.1007/11681878_14,soria2013optimal,geng2015staircase}, which produces LDP noise ranging from negative to positive infinity. In this work, they are referred to as ``unbounded mechanisms''.

\noindent
\textbf{Piecewise mechanism.}
Piecewise mechanism~\cite{wang2019collecting} produces the perturbed value $w^*$ of an original value $g_k\in[-1,1]$ following the distribution below:
\begin{equation*}
	\Pr(g_k^*)=
	\begin{cases}
		\frac{e^{\epsilon}-e^{\epsilon/2}}{2e^{\epsilon/2}+2}, &\mbox{if}\quad g_k^*\in\left[l(g_k),r(g_k)\right]\\
		\frac{1-e^{-\epsilon/2}}{2e^{\epsilon/2}+2},  &\mbox{if}\quad g_k^*\in\left[-Q,l(g_k))\cup(r(g_k),Q\right]
	\end{cases}
\end{equation*}
$Q=\frac{e^{\epsilon}+e^{\epsilon/2}}{e^{\epsilon}-e^{\epsilon/2}},l(g_k)=\frac{Q+1}{2} g_k-\frac{Q-1}{2},r(g_k)=l(g_k)+Q-1$.

In contrast to ``unbounded mechanisms'', Piecewise mechanism perturbs the original value into a bounded domain $[-Q,Q]$. Without loss of generality, such mechanisms are referred to as ``bounded mechanisms''.

\noindent
\textbf{Square wave mechanism.} This is yet another ``bounded'' LDP mechanism that improves Piecewise with more concentrated perturbation~\cite{li2020estimating}. Given any original value $g_k \in [0,1]$ and $b=\frac{\epsilon e^\epsilon-e^\epsilon+1}{2e^\epsilon(e^\epsilon-1-\epsilon)}$, the perturbed value $g_k^*\in [-b,b+1]$ follows the distribution as:
\begin{equation*}
	\Pr(g_k^*)=
	\begin{cases}
		\frac{e^\epsilon}{2be^\epsilon+1}, & \mbox{if } \left| g_k-g_k^*\right|<b\\
		\frac{1}{2be^\epsilon+1}, & \mbox{otherwise}
	\end{cases}
\end{equation*}
 
\noindent
\textbf{Gaussian mechanism.} Gaussian mechanism \cite{dwork2014algorithmic}, which instead follows the relaxed LDP, is proposed to address the low utility of the strict LDP. As another unbounded mechanism, given a value $g_k$ in the range of $[-1,1]$, the perturbed value is $g_k^*=g_k+Gau(0,8\ln \frac{1.25}{\delta}/\epsilon)$, where $Gau(\mu,\sigma^2)$ denotes a random variable that follows Gaussian distribution with probability density function $f(x)=\frac{1}{\sigma\sqrt{2\pi}}\exp(-\frac{(x-\mu)^2}{2\sigma^2})$.

Before analyzing the impact of LDP on FL, it is necessary to accurately model LDP noise regardless of LDP mechanisms. Based on a prior work \cite{duan2022utility}, we can model any LDP aggregation with a Gaussian distribution, as proven in Section \ref{sec::framework}.

\subsection{Federated Averaging and Optimization Techniques}
This work conducts analysis on the first and perhaps the most widely used FL algorithm, FedAvg (Federated Averaging)~\cite{mcmahan2017communication}. In FedAvg, the global objective is the weighted average of local objectives. Let $N$ denote the number of local devices, and each device possesses a local dataset $D_k (1\leq k\leq N)$. Then, we use $\boldsymbol{w}_k\left(1\leq k \leq N\right)$ to denote the local parameters (a.k.a the local model) in $k$-th local device. Given $S_k\subseteq D_k$ and $S_k=\left\{s_{k1}, s_{k2}, ..., s_{k(B-1)}, s_{kB}\right\}$ (where $B$ denotes the number of data in $S_k$), the local objective $F_k(\boldsymbol{w})$ can be formulated as $F_k(\boldsymbol{w};S_{k})=\frac{1}{B}\sum_{j=1}^{B} \mathit{l} (\boldsymbol{w};s_{kj})$, where $\mathit{l} (\boldsymbol{w};s_{kj})$ is the user-specified loss function trained on one subset data $s_{kj}$ to optimize $\boldsymbol{w}_k$. Given that $p_k$ is the weight of $k$-th device such that $p_k>0$ and $\sum_{k=1}^{N} p_k=1$, we consider the global optimization task: $	\min_{\boldsymbol{w}} \left\{F(\boldsymbol{w})=\sum_{k=1}^{N} p_k F_k(\boldsymbol{w};S_{k})\right\}$.

To optimize this task, we follow the common practice of existing works and use mini-batch stochastic gradient descent (SGD) \cite{lecun2002efficient} for further analysis and experiments. Given the total number of local iterations $T$, $\boldsymbol{w}_k^t=\left(\boldsymbol{w}_{k1}^t, \boldsymbol{w}_{k2}^t, ..., \boldsymbol{w}_{k(d-1)}^t, \boldsymbol{w}_{kd}^t\right)$ $\left(0\leq t\leq T-1\right)$ denotes a $d$-dimensional local weight vector (a.k.a the local model) derived from the $t$-th local iteration at the $k$-th local device (where $t=0$ is the initiate state). Besides, we use $\eta^t$ to denote the learning rate in the $t$-th local iteration. Then we have the gradient $\boldsymbol{g}^t_k$ of the $t$-th local iteration: $\boldsymbol{g}^t_k=\nabla F_k(\boldsymbol{w}^t_k;S_k)$
%\begin{equation}
%	\begin{aligned}
%	\boldsymbol{g}^t_k=\nabla F_k(\boldsymbol{w}^t_k;S_k),
%	\end{aligned}	
%\label{equ::graident}
%\end{equation}
, where $\nabla F_k(\boldsymbol{w})=\left(\frac{F_k}{\partial \boldsymbol{w}_{1}}, \frac{F_k}{\partial \boldsymbol{w}_{2}}, ..., \frac{F_k}{\partial \boldsymbol{w}_{d-1}}, \frac{F_k}{\partial \boldsymbol{w}_{d}}\right)$. Given $\nabla_k^t=\nabla F_k(\boldsymbol{w}_k^t;D_k)$, we have $\mathbb{E}(\boldsymbol{g}^t_k)=\mathbb{E}(F_k(\boldsymbol{w}_k^t;S_k))=\nabla_k^t$. The $t$-th local iteration updates local weight $\boldsymbol{w}_k^{t+1}$ as $\boldsymbol{w}_k^{t+1}=\boldsymbol{w}_k^t-\eta^t \boldsymbol{g}_k^t$.
%\begin{equation}
%	\boldsymbol{w}_k^{t+1}=\boldsymbol{w}_k^t-\eta^t \boldsymbol{g}_k^t
%\label{equ::GradientDescent}
%\end{equation}

By tuning the local batch size $B$, the analysis on this optimization technique also applies to its variants. For example, if $B=\left|D_k\right|$, it is equivalent to the batch gradient descent \cite{boyd_vandenberghe_2004}; if $B=1$, it is equivalent to the stochastic gradient descent \cite{bottou2012stochastic}. Throughout this paper, we abbreviate mini-batch stochastic gradient descent and its variants collectively as SGD.

SGD is known to have an intrinsic problem of gradient explosion \cite{pascanu2013difficulty}. It often occurs when the gradients become very large during backpropagation, and causes the model to converge rather slowly or not to converge at all. As the most effective solution to this problem, gradient clipping \cite{pascanu2013difficulty} is also considered in this work. Let $\left\|\boldsymbol{g}\right\|$ denote the $L_2$-norm of a $d$-dimensional vector $\boldsymbol{g}=(\boldsymbol{g}_1, \boldsymbol{g}_2, ..., \boldsymbol{g}_{d-1}, \boldsymbol{g}_d)$, i.e., $\left\|\boldsymbol{g}\right\|=\sqrt{\sum_{z=1}^{d}\boldsymbol{g}_z^2}$. Assume that $G$ is the maximum $L_2$-norm value of all possible gradients for any weight $\boldsymbol{w}_k$ derived from any subset $S_k$, i.e., $G=\sup_{\boldsymbol{w}_k\in \mathbb{R}^d, S_k\in D_k}\mathbb{E}\left[\left\|\boldsymbol{g}_k\right\|\right]$. Then each local gradient $\boldsymbol{g}_k^t$ is clipped by a clipping threshold $C\in \left(0,G\right]$. Formally, $	\tilde{\boldsymbol{g}}_k^t=\frac{\boldsymbol{g}_k^t}{\max \left\{1,\left\|\boldsymbol{g}_k^t\right\|/C\right\}}$. On this basis, we derive the updated weight $\boldsymbol{w}_k^{t+1}$ with the clipped gradient from the $t$-th local iteration as $\boldsymbol{w}_k^{t+1}=\boldsymbol{w}_k^t-\eta^t \tilde{\boldsymbol{g}}_k^t$.
%\begin{equation}
%	\boldsymbol{w}_k^{t+1}=\boldsymbol{w}_k^t-\eta^t \tilde{\boldsymbol{g}}_k^t
%\label{equ::ClippedGD}
%\end{equation}

\subsection{Problem Formulation of Federated LDP-SGD}
Without loss of generality, we consider FedAvg under SGD with LDP noise. Before global aggregation, $\boldsymbol{w}_k^{t+1}$ is perturbed to $\boldsymbol{w}_k^{{t+1}*}$ by adding LDP noise $\boldsymbol{n}_k^t$ to $\tilde{\boldsymbol{g}}_k^t$, before being sent to the central server. Let $\boldsymbol{g}_k^{t*}$ denote the perturbed local gradient. Formally, $\boldsymbol{g}_k^{t*}=\tilde{\boldsymbol{g}}_k^t+\boldsymbol{n}_k^t$. On receiving local perturbed models from all devices, the central server aggregates them to obtain the current global model $\boldsymbol{w}^{t+1*}$.
Suppose there exists a global optima $\boldsymbol{w}^{\star}$, the convergence can be measured by the Euclidean Distance between the current global model $\boldsymbol{w}^{t+1*}$ and the optima $F(\boldsymbol{w}^{\star})$. Formally, $\mbox{Convergence Rate}=\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^{\star}\right\|^2$.


The problem in this work is to investigate the impact of LDP noise $\left\{\boldsymbol{n}_k^t|1\leq k\leq N\right\}$ on global convergence $\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^{\star}\right\|^2$, and further improve the convergence rate by reducing the negative impact of LDP perturbation. 
%\begin{algorithm}[H]
%	\caption{FedAvg under LDP-SGD}
%	\label{alg:FedAvgLDPSGD}
%	\begin{algorithmic}[1]
%		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
%		\renewcommand{\algorithmicensure}{\textbf{Output:}}
%		\REQUIRE initiate global model $\boldsymbol{w}^0$, LDP noise $\boldsymbol{n}_k^t$, training rounds $T/E$, local dataset $D_k$, learning rate $\eta^t$.
%		\ENSURE  the updated global model $\boldsymbol{w}^{t+1*}$.
%		\STATE Initialize global model parameters $\boldsymbol{w}^0$.
%		\FOR{each round $T/E = 1, 2, \ldots$}
%		%	\STATE Randomly select a subset of clients $C_t \subseteq C$
%		\FOR{each local device $k$}
%		\STATE Send current global updates $\boldsymbol{w}^t$ to device $k$.
%		\STATE Device $k$ trains a local model with SGD on its dataset $D_k$ using $\boldsymbol{w}^t_k$, and obtains the local perturbed model $\boldsymbol{w}_k^{t+1*}=\boldsymbol{w}_k^t-\eta^t(\tilde{\boldsymbol{g}}+\boldsymbol{n}_k^t)$.
%		\STATE Send local perturbed update $\boldsymbol{w}_k^{t+1*}$ to the server.
%		\ENDFOR
%		\STATE Server aggregates the local models using a weighted average: $\boldsymbol{w}^{t+1*} = \sum_{k=1}^{N} p_k \boldsymbol{w}_k^{t+1*}$.
%		\ENDFOR
%	\end{algorithmic}
%\end{algorithm}

==> sec/0_abstract.tex <==
\begin{abstract}
We propose a geometric perturbation strategy to optimize differentially private stochastic gradient descent (DP-SGD). Differential privacy (DP), which protects sensitive data in training datasets, has emerged as a prevalent privacy preservation scheme in a wide variety of machine learning and deep learning tasks, such as DP-SGD. However, DP-SGD normally performs poorly under complex models, due to the obfuscated training process incurred by DP noise. Although there exist ample works on reducing the noise scale (e.g., adaptive clipping to reduce the sensitivity of a gradient, amplifying the privacy bounds to save privacy budgets, introducing more efficient SGD techniques into DP and training a model across various datasets collaboratively), there is still much room for improvements. 

In our work, our theoretical analysis first reveals that the direction of the perturbed gradient, rather than the magnitude, is much more significant for the efficient descent. Inspired by this, we then design a geometric perturbation strategy GeoDP within the DP framework, which perturbs the direction of a gradient less than the traditional DP-SGD so as to achieve better model efficiency. Orthogonal to all existing optimization techniques, this design provides a geometric perspective to mitigate the negative impact of DP noise on SGD. We conduct extensive experiments on two public datasets (i.e., CIFAR-10 and MNIST) and two prevalent models (i.e., logistic regression and CNN), to confirm the effectiveness of our strategy.
\end{abstract}

==> strategy.tex <==
\section{LDPVec: Enhancing Federated LDP-SGD from A Geometric Perspective}
\label{sec::stra}
In our framework, we observe that LDP noise can sometimes speedup the convergence, rather than only slowing it. In this section, we seize this opportunity to {\bf rearrange the direction of the LDP noise}, so that the convergence can be speedup while providing the same level of LDP protection. The rationale of targeting at the direction is that the relative angle between the gradient descent and the LDP noise dictates the impact of the LDP noise on the convergence, as indicated by Item B. Instead of only perturbing the local gradient as numeric values in existing works, our strategy, without changing the underlying LDP mechanism, perturbs both the magnitude and the direction of the local gradient to make positive impact of LDP noise to the convergence. As such, this strategy is orthogonal to all existing LDP mechanisms and LDP-SGD optimizations.

In what follows, we first introduce $d$-spherical coordinate system \cite{thomas2006multivariable}, where a $d$-dimensional gradient is converted to one magnitude and one direction. By perturbing local gradients in such a system, we propose our perturbation strategy \textit{LDPVec} to enhance the global convergence. Rigorous analysis is provided to prove its compliance with LDP definition and huge advantage over numerical perturbation.

\subsection{Hyper-spherical Coordinate System}
The $d$-spherical coordinate system, also known as the hyper-spherical coordinate system, is commonly used to analyze geometric objects in high-dimensional space, e.g., the gradient. Compared to the rectangular coordinate system \cite{thomas2006multivariable}, such system directly represents any $d$-dimensional vector  $\boldsymbol{g}=(\boldsymbol{g}_1, \boldsymbol{g}_2, ..., \boldsymbol{g}_{d-1}, \boldsymbol{g}_d)$ using a magnitude $\left\|\boldsymbol{g}\right\|$ and a direction $\boldsymbol{\theta}=\left(\boldsymbol{\theta}_1,\boldsymbol{\theta}_2,...,\boldsymbol{\theta}_{d-2},\boldsymbol{\theta}_{d-1}\right)$. Formally, the magnitude is:
\begin{equation}
	\left\|\boldsymbol{g}\right\|=\sqrt{\sum_{z=1}^{d}\boldsymbol{g}_z^2}
\label{equ::SphMig}
\end{equation}
and its direction $\boldsymbol{\theta}$ is:
\begin{equation}
\begin{aligned}
	\boldsymbol{\theta}_z=
	\begin{cases}
		\arctan{\frac{\sqrt{\sum_{z}^{d}\boldsymbol{g}_{z+1}^2}}{\boldsymbol{g}_z}}, &\mbox{if }1\leq z\leq d-2\\
		\pi-2\arctan\left(\frac{\boldsymbol{g}_z+\sqrt{\boldsymbol{g}_z^2+\boldsymbol{g}_{z+1}^2}}{\boldsymbol{g}_{z+1}}\right), &\mbox{if }z=d-1
	\end{cases}
\end{aligned}
\label{equ::SphAng}
\end{equation}

Given a vector $\left(\left\|\boldsymbol{g}\right\|, \boldsymbol{\theta}\right)$ in $d$-spherical coordinates, we can also convert it back to rectangular coordinates $(\boldsymbol{g}_1, \boldsymbol{g}_2, ..., \boldsymbol{g}_{d-1}, \boldsymbol{g}_d)$ using the following equation:
\begin{equation}
\begin{aligned}
	\boldsymbol{g}_z =
	\begin{cases}
		\left\|\boldsymbol{g}\right\| \cos{\boldsymbol{\theta}_z},  & \mbox{if }\ z=1 \\
		\left\|\boldsymbol{g}\right\| \sin{\boldsymbol{\theta}_1} \sin{\boldsymbol{\theta}_2} \dots \sin{\boldsymbol{\theta}_{z-1}} \cos{\boldsymbol{\theta}_z}, &\mbox{if }\ 2 \leq z \leq d - 1\\
		\left\|\boldsymbol{g}\right\| \sin{\boldsymbol{\theta}_1} \sin{\boldsymbol{\theta}_2} \dots \sin{\boldsymbol{\theta}_{z-2}} \sin{\boldsymbol{\theta}_{z-1}}, &\mbox{if }\ z=d
	\end{cases}
\end{aligned}
\label{equ::Rec}
\end{equation}
%Figure \ref {fig::hyper} provides an example of conversions in three-dimensional space. 
Without loss of generality, we use $\boldsymbol{g}\leftrightarrow\left(\left\|\boldsymbol{g}\right\|, \boldsymbol{\theta}\right)$ to denote the reversible conversions between two systems.
%\begin{figure}[htbp]
%	\centering
%	\includegraphics[width=0.4\linewidth]{figure/illustration/hypersphere.pdf}
%	\caption{Coordinates Conversions in Three-dimensional Space.}
%	\label{fig::hyper}
%\end{figure}
\subsection{LDPVec---LDP Perturbation Vectorization for Federated LDP-SGD}
\label{subsec::LDPVec}
While existing works implement numerical perturbation in the rectangular coordinate system, our perturbation strategy \textit{LDPVec} instead mitigates the negative impact of LDP via $d$-spherical coordinate system. As shown in Algorithm \ref{alg:LDPVec}, \textit{LDPVec} perturbs the local gradient in four steps. Before the global update, the local device first derives the noise-free local model (Step \ref{item::GradientDescent}). Then, both the noise-free local model and the clipped local gradient are converted into a $d$-spherical coordinate system (Step \ref{item::Sph}). Afterwards, a LDP mechanism perturbs the magnitude of the local gradient and the direction of the noise-free local model, respectively (Step \ref{item::Per}). Finally, the perturbed gradient, including the perturbed magnitude of the clipped gradient and the perturbed direction of the noise-free local model, is converted from $d$-spherical coordinate system (Step \ref{item::Rec}). 

The main challenges lie in two folds. First, no existing works prove that the conversion in Step \ref{item::Per} can still satisfy LDP. Second, it is theoretically unclear whether a vectorized perturbation is superior to the numerical one for gradients. To address the first challenge, we establish the following lemma to confirm that the conversion between coordinate systems does not change the LDP preservation.
\begin{algorithm}[H]
	\caption{LDPVec}
	\label{alg:LDPVec}
	\begin{algorithmic}[1]
		\renewcommand{\algorithmicrequire}{\textbf{Input:}}
		\renewcommand{\algorithmicensure}{\textbf{Output:}}
		\REQUIRE local model $\boldsymbol{w}_k^t$ of the current state, learning rate $\eta^t$, the LDP mechanism $\mathcal{M}$, local clipped gradient $\tilde{\boldsymbol{g}}_k^t$, privacy budget $\epsilon_1$ and $\epsilon_2$, probability $\delta_1$ and $\delta_2$.
		\ENSURE  perturbed gradient $\boldsymbol{g}_k^{t\star}$.
		\STATE Calculate $\boldsymbol{w}_k^{t+1}=\boldsymbol{w}_k^t-\eta^t\tilde{\boldsymbol{g}}_k^t$.
		\label{item::GradientDescent}
		\STATE Convert $\tilde{\boldsymbol{g}}_k^t$ and  $\boldsymbol{w}_k^{t+1}$ to $d$-spherical coordinates as $\left(\left\|\tilde{\boldsymbol{g}}_k^t\right\|, \boldsymbol{\theta}_1\right)$ and $\left(\left\|\boldsymbol{w}_k^{t+1}\right\|, \boldsymbol{\theta}_2\right)$, respectively, according to Equation \ref{equ::SphMig} and Equation \ref{equ::SphAng}.
		\label{item::Sph}
		\STATE
		$\left\|\tilde{\boldsymbol{g}}_k^{t}\right\|^*=\mathcal{M}\left(\left\|\tilde{\boldsymbol{g}}_k^t\right\|,\epsilon_1,\delta_1\right)$,
		$\boldsymbol{\theta}_2^*=\mathcal{M}(\boldsymbol{\theta}_2,\epsilon_2,\delta_2)$.
		\label{item::Per}
		\STATE Convert $\left(\left\|\tilde{\boldsymbol{g}}_k^{t}\right\|^*,\boldsymbol{\theta}_2^*\right)$ back to rectangular coordinates as the perturbed gradient $\boldsymbol{g}_k^{t\star}$, according to Equation \ref{equ::Rec}.
		\label{item::Rec}
	\end{algorithmic}
\end{algorithm}

\begin{lemma}
	 Given any LDP mechanism $\mathcal{M}$ and $\boldsymbol{g}\leftrightarrow\left(\left\|\boldsymbol{g}\right\|, \boldsymbol{\theta}\right)$, $\boldsymbol{g}^*=M(\boldsymbol{g})$ is $(\epsilon_1+\epsilon_2,\delta_1+\delta_2)$-locally differentially private if $\left\|\boldsymbol{g}\right\|^*=M(\left\|\boldsymbol{g}\right\|)$ and $\boldsymbol{\theta}^*=M(\boldsymbol{\theta})$ are $(\epsilon_1,\delta_1)$- and $(\epsilon_2,\delta_2)$-locally differentially private, respectively.
\label{lem::CoordinateConversion}
\end{lemma}
\begin{proof}
For any three pairs of $\boldsymbol{g}_i,\boldsymbol{g}_j$, $\left\|\boldsymbol{g}\right\|_i,\left\|\boldsymbol{g}\right\|_j$ and $\boldsymbol{\theta}_i,\boldsymbol{\theta}_j$, we have:
\begin{equation}
\begin{aligned}
	&\Pr(\mathcal{M}(\boldsymbol{g}_i)=\boldsymbol{g}^*)=\Pr\left(\mathcal{M}(\left\|\boldsymbol{g}\right\|_i)=\left\|\boldsymbol{g}\right\|^*,\mathcal{M}(\boldsymbol{\theta}_i)=\boldsymbol{\theta}^*\right)\\&=\Pr\left(\mathcal{M}(\left\|\boldsymbol{g}\right\|_i)=\left\|\boldsymbol{g}\right\|^*\right)\Pr\left(\mathcal{M}(\boldsymbol{\theta}_i)=\boldsymbol{\theta}^*\right)\\&\leq  1\land\left(e^{\epsilon_1}\Pr\left(\mathcal{M}(\left\|\boldsymbol{g}\right\|_j)=\left\|\boldsymbol{g}\right\|^*\right)+\delta_1\right) \Pr\left(\mathcal{M}(\boldsymbol{\theta}_i)=\boldsymbol{\theta}^*\right)\\&\leq \left(1\land e^{\epsilon_1}\Pr\left(\mathcal{M}(\left\|\boldsymbol{g}\right\|_j)=\left\|\boldsymbol{g}\right\|^*\right)+\delta_1\right) \Pr\left(\mathcal{M}(\boldsymbol{\theta}_i)=\boldsymbol{\theta}^*\right)\\&\leq \left(1\land \left(e^{\epsilon_1}\Pr\left(\mathcal{M}(\left\|\boldsymbol{g}\right\|_j)=\left\|\boldsymbol{g}\right\|^*\right)\right)\right)\Pr\left(\mathcal{M}(\boldsymbol{\theta}_i)=\boldsymbol{\theta}^*\right)+\delta_1
\end{aligned}
\label{equ::CoordinateConversion1}
\end{equation}
Note that $\Pr\left(\mathcal{M}(\boldsymbol{\theta}_i)=\boldsymbol{\theta}^*\right)\leq e^{\epsilon_2}\Pr\left(\mathcal{M}(\boldsymbol{\theta}_j)=\boldsymbol{\theta}^*\right)+\delta_2$. By applying this to Equation \ref{equ::CoordinateConversion1}, we have:
\begin{equation}
	\begin{aligned}
		\Pr(\mathcal{M}(\boldsymbol{g}_i)=\boldsymbol{g}^*)\leq& \Pr(\mathcal{M}(\left\|\boldsymbol{g}\right\|_j)=\left\|\boldsymbol{g}\right\|^*)\Pr\left(\mathcal{M}(\boldsymbol{\theta}_j)=\boldsymbol{\theta}^*\right)\\&e^{\epsilon_1}e^{\epsilon_2}+ \delta_1+\delta_2\\\leq& e^{\epsilon_1+\epsilon_2}\Pr(\mathcal{M}(\boldsymbol{g}_j)=\boldsymbol{g}^*)+(\delta_1+\delta_2)
	\end{aligned}
	\label{equ::CoordinateConversion}
\end{equation}
by which this lemma is proven.
\end{proof}
Also, in this following lemma we prove that protecting the direction of the local model is equivalent to protecting the direction of the local gradient.
\begin{lemma}
	Given any LDP mechanism $\mathcal{M}$, $\boldsymbol{g}\leftrightarrow\left(\left\|\boldsymbol{g}\right\|, \boldsymbol{\theta}_g\right)$ and $\boldsymbol{w}\leftrightarrow\left(\left\|\boldsymbol{w}\right\|,
	 \boldsymbol{\theta}_w\right)$, $\left\|\boldsymbol{w}\right\|^*=\mathcal{M}(\left\|\boldsymbol{w}\right\|,\epsilon_1,\delta_1)$ while $\left\|\boldsymbol{g}\right\|^*=\mathcal{M}(\left\|\boldsymbol{g}\right\|,\epsilon_1,\delta_1)$. Let $\boldsymbol{g}$ be the linear mapping of $\boldsymbol{w}$, and $\boldsymbol{\theta}_g^*$ be the noisy version of $\boldsymbol{\theta}_g$. Then $\boldsymbol{\theta}_g^*$ is also $(\epsilon_2,\delta_2)$-locally differently private if $\boldsymbol{\theta}_w^*=\mathcal{M}(\boldsymbol{\theta}_w)$ is $(\epsilon_2,\delta_2)$-locally differently private.
\label{lem::Equivalency}	
\end{lemma}
\begin{proof}
Now that $\mathcal{M}(\left\|\boldsymbol{w}\right\|)$ and $\mathcal{M}(\boldsymbol{\theta}_w)$ are $(\epsilon_1,\delta_1)$- and $(\epsilon_2,\delta_2)$-locally differentially private, we have $\mathcal{M}(\boldsymbol{w})$ is $(\epsilon_1+\epsilon_2,\delta_1+\delta_2)$-locally differentially private, according to Lemma \ref{lem::CoordinateConversion}. From Lemma \ref{lem::linear}, $\mathcal{M}(\boldsymbol{g})$ is also $(\epsilon_1+\epsilon_2,\delta_1+\delta_2)$-locally differentially private because $\boldsymbol{g}$ is the linear mapping of $\boldsymbol{w}$. Since $\mathcal{M}(\left\|\boldsymbol{g}\right\|)$ is $(\epsilon_1,\delta_1)$-locally differentially private, Lemma \ref{lem::CoordinateConversion} proves that $\mathcal{M}(\boldsymbol{\theta}_g)$ is $(\epsilon_1+\epsilon_2-\epsilon_1=\epsilon_2,\delta_1+\delta_2-\delta_1=\delta_2)$-locally differentially private, by which this lemma is proven.
\end{proof}
Since the local gradient is a linear mapping of the local model (i.e., $\boldsymbol{w}_k^{t+1}=\boldsymbol{w}_k^t-\eta^t\tilde{\boldsymbol{g}}_k^t$), protecting the direction of local gradient is equivalent to protecting the local model, according to Lemma \ref{lem::Equivalency}. 

As for the second challenge, the following theorem confirms the superiority of our perturbation strategy over existing numerical perturbations.
\begin{theorem}
Let $\boldsymbol{w}^{t+1\star}=\sum_{k=1}^{N}p_k (\boldsymbol{w}_k^t-\eta^t\tilde{\boldsymbol{g}}^{t\star}_k)$ and $\boldsymbol{w}^{t+1*}=\sum_{k=1}^{N}p_k (\boldsymbol{w}_k^t-\eta^t\tilde{\boldsymbol{g}}^{t*}_k)$. The following inequality always holds if $\tilde{\boldsymbol{g}}^{t\star}_k$ and $\tilde{\boldsymbol{g}}^{t*}_k$ are both $(\epsilon_1+\epsilon_2,\delta_1+\delta_2)$-locally differentially private:
\begin{equation*}
  \mathbb{E}\left(\left\|\boldsymbol{w}^{t+1\star}-\boldsymbol{w}^\star\right\|^2\right)<\mathbb{E}\left(\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^\star\right\|^2\right)
\vspace{-0.2in}
\end{equation*}
\label{the::Superiority}
\end{theorem}
\begin{proof}
Lemma \ref{lem::CoordinateConversion} establishes that the conversion between coordinate systems does not change the level of privacy preservation. Given $\boldsymbol{g}_k^t\leftrightarrow\left(\left\|\boldsymbol{g}_k^t\right\|, \boldsymbol{\theta}_k^t\right)$, the existing numerical perturbation $\tilde{\boldsymbol{g}}_k^{t*}=\mathcal{M}(\tilde{\boldsymbol{g}}_k^t,\epsilon_1+\epsilon_2,\delta_1+\delta_2)$ can be decomposed of $\left\|\tilde{\boldsymbol{g}}_k^{t}\right\|^*=\mathcal{M}\left(\left\|\tilde{\boldsymbol{g}}_k^t\right\|,\epsilon_1,\delta_1\right)$ and	$\boldsymbol{\theta}_k^{t*}=\mathcal{M}(\boldsymbol{\theta}_1,\epsilon_2,\delta_2)$, while $\tilde{\boldsymbol{g}}^{t\star}_k$ can be decomposed of $\left\|\tilde{\boldsymbol{g}}_k^{t}\right\|^*=\mathcal{M}\left(\left\|\tilde{\boldsymbol{g}}_k^t\right\|,\epsilon_1,\delta_1\right)$ and	$\boldsymbol{\theta}_k^{t'*}=\mathcal{M}(\boldsymbol{\theta}_k^{t'},\epsilon_2,\delta_2)$, according to Algorithm \ref{alg:LDPVec}. Note that $\boldsymbol{\theta}_k^{t'}$ is the direction of $\boldsymbol{w}_k^t-\eta^t\tilde{\boldsymbol{g}}^{t}_k$. According to Equation \ref{equ::difference}, for $\tilde{\boldsymbol{g}}_k^{t*}$, we have:
\begin{equation*}
\begin{aligned}
	&\mathbb{E}(\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^\star\right\|^2)-\mathbb{E}(\left\|\boldsymbol{w}^{t+1}-\boldsymbol{w}^\star\right\|^2)\\=&\mathbb{E}\left(-2\langle\boldsymbol{w}^t-\eta^t\tilde{\boldsymbol{g}}^t,\boldsymbol{n}^{t}\rangle+{\eta^t}^2{\boldsymbol{n}^{t}}^2+2\langle\boldsymbol{w}^\star,\boldsymbol{n}^{t}\rangle\right)\\\leq&-2\min_{\tilde{\boldsymbol{g}}_k^t}\left(\left\|\boldsymbol{w}_k^t-\eta^t\tilde{\boldsymbol{g}}_k^t\right\|\left\|\tilde{\boldsymbol{g}}_k^{t}\right\|^*\right)\mathbb{E}(\cos(\boldsymbol{\theta}))+{\eta^t}^2\left\|\tilde{\boldsymbol{g}}_k^{t}\right\|^{*2}+2\langle\boldsymbol{w}^\star,\boldsymbol{n}^{t}_k\rangle
\end{aligned}
\end{equation*}
and for $\tilde{\boldsymbol{g}}_k^{t\star}$, we have:
\begin{equation*}
	\begin{aligned}
		&\mathbb{E}(\left\|\boldsymbol{w}^{t+1\star}-\boldsymbol{w}^\star\right\|^2)-\mathbb{E}(\left\|\boldsymbol{w}^{t+1}-\boldsymbol{w}^\star\right\|^2)\\\leq&-2\min_{\tilde{\boldsymbol{g}}_k^t}\left(\left\|\boldsymbol{w}_k^t-\eta^t\tilde{\boldsymbol{g}}_k^t\right\|\left\|\tilde{\boldsymbol{g}}_k^{t}\right\|^*\right)\mathbb{E}(\cos(\boldsymbol{\theta}'))+{\eta^t}^2\left\|\tilde{\boldsymbol{g}}_k^{t}\right\|^{*2}+2\langle\boldsymbol{w}^\star,\boldsymbol{n}^{t}_k\rangle
	\end{aligned}
\end{equation*}
where $\boldsymbol{\theta}$ and $\boldsymbol{\theta}'$ denote the angles between respective noise and the local model. Therefore, we have $\mathbb{E}(\cos(\boldsymbol{\theta}))<\mathbb{E}(\cos(\boldsymbol{\theta}'))$. If $t$ is not sufficiently large, $\boldsymbol{w}^{t+1}$ will be far away from $\boldsymbol{w}^\star$, so $2\langle\boldsymbol{w}^\star,\boldsymbol{n}^{t}\rangle$ will become negligible. Therefore, we have:
\begin{equation}
\begin{aligned}
		&\mathbb{E}(\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^\star\right\|^2)-\mathbb{E}(\left\|\boldsymbol{w}^{t+1}-\boldsymbol{w}^\star\right\|^2)\\\leq&-2\min_{\tilde{\boldsymbol{g}}_k^t}\left(\left\|\boldsymbol{w}_k^t-\eta^t\tilde{\boldsymbol{g}}_k^t\right\|\left\|\tilde{\boldsymbol{g}}_k^{t}\right\|^*\right)\mathbb{E}(\cos(\boldsymbol{\theta}))+{\eta^t}^2\left\|\tilde{\boldsymbol{g}}_k^{t}\right\|^{*2}
\end{aligned}
\label{equ::SupNum}
\end{equation}
and
\begin{equation}
	\begin{aligned}
		&\mathbb{E}(\left\|\boldsymbol{w}^{t+1\star}-\boldsymbol{w}^\star\right\|^2)-\mathbb{E}(\left\|\boldsymbol{w}^{t+1}-\boldsymbol{w}^\star\right\|^2)\\\leq&-2\min_{\tilde{\boldsymbol{g}}_k^t}\left(\left\|\boldsymbol{w}_k^t-\eta^t\tilde{\boldsymbol{g}}_k^t\right\|\left\|\tilde{\boldsymbol{g}}_k^{t}\right\|^*\right)\mathbb{E}(\cos(\boldsymbol{\theta}'))+{\eta^t}^2\left\|\tilde{\boldsymbol{g}}_k^{t}\right\|^{*2}
	\end{aligned}
\label{equ::SupVec}
\end{equation}
By subtracting Equation \ref{equ::SupNum} from Equation \ref{equ::SupVec}, we have:
\begin{equation}
	\mathbb{E}(\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^\star\right\|^2)<\mathbb{E}(\left\|\boldsymbol{w}^{t+1\star}-\boldsymbol{w}^\star\right\|^2)
\label{equ::FiSuper}
\end{equation}
%If $t\to\infty$, $\boldsymbol{w}^t-\eta^t\tilde{\boldsymbol{g}}^t\to\boldsymbol{w}^\star$. Then, we have:
%\begin{equation}
%	\begin{aligned}
%		&\mathbb{E}(\left\|\boldsymbol{w}^{t+1*}-\boldsymbol{w}^\star\right\|^2)-\mathbb{E}(\left\|\boldsymbol{w}^{t+1}-\boldsymbol{w}^\star\right\|^2)\\=&\mathbb{E}\left(-2\langle\boldsymbol{w}^t-\eta^t\tilde{\boldsymbol{g}}^t,\boldsymbol{n}^{t}\rangle+{\eta^t}^2{\boldsymbol{n}^{t}}^2+2\langle\boldsymbol{w}^\star,\boldsymbol{n}^{t}\rangle\right)={\eta^t}^2\left\|\tilde{\boldsymbol{g}}_k^{t}\right\|^{*2}\\=&\mathbb{E}(\left\|\boldsymbol{w}^{t+1\star}-\boldsymbol{w}^\star\right\|^2)-\mathbb{E}(\left\|\boldsymbol{w}^{t+1}-\boldsymbol{w}^\star\right\|^2)
%	\end{aligned}
%\label{equ::InfSuper}
%\end{equation}
%By Equations \ref{equ::FiSuper} and \ref{equ::InfSuper}, this theorem is proved. 
by which this theorem is proven
\end{proof}

Theorem \ref{the::Superiority} proves that the convergence of federated LDP-SGD under vectorized perturbation is always superior to that under existing numerical perturbation in terms of the expected convergence distance. Basically, there are two major reasons to explain the superiority. First, compared with existing perturbation, LDPVec can perturb the magnitude and the direction of a gradient, respectively. From the perspective of utility, \textbf{LDPVec can align the direction of LDP noise $\boldsymbol{n}^{t}_k$ towards the direction of the local model $\boldsymbol{w}_k^t-\eta^t\tilde{\boldsymbol{g}}^{t}_k$, which speedups the convergence of LDP-SGD}, as proven by Equation \ref{equ::FiSuper}. Meanwhile, the privacy preservation of LDPVec is the same as the existing perturbation, as verified by Lemma \ref{lem::Equivalency}. Second, LDPVec has a intrinsic advantage, i.e., the direction has a much smaller range than numerical values. While numerical values of a gradient usually range from $(-\infty,\infty)$, the range of angles in LDPVec is $[0,2\pi]$. Therefore, \textbf{the noise scale of LDPVec is naturally smaller than that of numerical perturbation, even under the same LDP preservation.} Although the clipping techniques can can reduce noise scale of numerical perturbation, they can also help LDPVec to make more moderate perturbation, as verified in Section \ref{sec::exp}.

Overall, the hyper-spherical coordinate system, which represents any vector by a magnitude and a direction, allows us to align the direction of LDP noise to towards that of the local model, while still retaining the same privacy preservation. 
